SparseP: Towards Efficient Sparse Matrix Vector Multiplication on Real Processing-In-Memory Systems

Several manufacturers have already started to commercialize near-bank Processing-In-Memory (PIM) architectures. Near-bank PIM architectures place simple cores close to DRAM banks and can yield significant performance and energy improvements in parallel applications by alleviating data access costs. Real PIM systems can provide high levels of parallelism, large aggregate memory bandwidth and low memory access latency, thereby being a good fit to accelerate the widely-used, memory-bound Sparse Matrix Vector Multiplication (SpMV) kernel. This paper provides the first comprehensive analysis of SpMV on a real-world PIM architecture, and presents SparseP, the first SpMV library for real PIM architectures. We make three key contributions. First, we implement a wide variety of software strategies on SpMV for a multithreaded PIM core and characterize the computational limits of a single multithreaded PIM core. Second, we design various load balancing schemes across multiple PIM cores, and two types of data partitioning techniques to execute SpMV on thousands of PIM cores: (1) 1D-partitioned kernels to perform the complete SpMV computation only using PIM cores, and (2) 2D-partitioned kernels to strive a balance between computation and data transfer costs to PIM-enabled memory. Third, we compare SpMV execution on a real-world PIM system with 2528 PIM cores to state-of-the-art CPU and GPU systems to study the performance and energy efficiency of various devices. SparseP software package provides 25 SpMV kernels for real PIM systems supporting the four most widely used compressed matrix formats, and a wide range of data types. Our extensive evaluation provides new insights and recommendations for software designers and hardware architects to efficiently accelerate SpMV on real PIM systems.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> backup/backup1/0-abstract.tex <==

\begin{abstract}

Several manufacturers have already started to commercialize near-bank Processing-in-Memory (PIM) architectures, after decades of research efforts. Near-bank PIM architectures place simple cores close to DRAM banks. Recent research demonstrates that they can yield significant performance and energy improvements in parallel applications by alleviating data access costs.
%They represent a promising way to alleviate data movement costs. \jgl{Not just promising. Several works have shown the benefits of these real PnM architectures.} 
Real PIM systems can provide high levels of parallelism and large aggregate memory bandwidth and low memory access latency, thereby being a good fit to accelerate the Sparse Matrix Vector Multiplication (\spmv{}) kernel. \spmv{} has been characterized as one of the most significant and thoroughly
studied computational scientific kernels, and it is primarily a memory-bound kernel posing intense memory accesses due its algorithmic nature, the compressed matrix format used, and the sparsity patterns of the input matrices given. 
%\jgl{Mention how important SpMV is.}. 




This paper provides the first comprehensive analysis of \spmv{} on a real-world PIM architecture, and presents \SparseP{}, the first \spmv{} library for real PIM architectures. We make three key contributions. First, we implement a wide variety of software strategies on \spmv{} for a multithreaded PIM core, including (1) various compressed matrix formats, (2) load balancing schemes among parallel threads and (3) synchronization approaches, and characterize the computational limits of a single multithreaded PIM core. %evaluate the compute capabilities of a simple multithreaded PIM core \jgl{Not clear what you mean here}. 
Second, we design various load balancing schemes among multiple PIM cores, and two types of data partitioning techniques to execute \spmv{} on thousand PIM cores: (1) 1D partitioning kernels to perform the complete \spmv{} computation only using PIM cores %to produce the final output vector using only PIM cores 
and (2) 2D partitioning kernels to strive a balance between computation and data transfer costs to PIM-enabled memory.
%(1) 1D partitioning kernels to offload the whole \spmv{} execution to multiple PIM cores and (2) 2D partitioning kernels to strive a balance between computation and data transfer costs to PIM-enabled memory. %\jgl{For me, second and third are the same: partitioning strategies, each with its advantages.} 
Finally, we compare the \spmv{} execution on a real-world PIM system with 2528 PIM cores to an Intel Xeon CPU and an NVIDIA Tesla V100 GPU to study the performance and energy efficiency of various devices, i.e., both memory-centric PIM systems and conventional processor-centric CPU/GPU systems for the \spmv{} kernel.
%\jgl{What is the goal of the comparison? Identify improvement points for PIM architectures?}. 
\SparseP{} software package provides 25 \spmv{} kernels for real PIM systems supporting the four most widely used compressed matrix formats, i.e., CSR, COO, BCSR and BCOO, %\jgl{Say which ones.} 
and a wide range of data types. \SparseP{} is publicly and freely available. Our extensive evaluation using 26 matrices with various sparsity patterns provides new insights and recommendations for software designers and hardware architects to efficiently accelerate the \spmv{} kernel on real PIM systems.



\end{abstract}


==> backup/backup1/1-introduction.tex <==

\section{Introduction} 
%\jgl{Revise order of keywords above. For example, SpMV should go before DRAM, real-system characterization...}

Sparse Matrix-Vector Multiplication (\spmv) is a fundamental linear algebra kernel for important applications from the scientific computing, machine learning, and graph analytics domains. In commodity systems, it has been repeatedly reported to achieve only a small fraction of the peak performance~\cite{Elafrou2018SparseX,Yan2014YaSpMV,Liu2018Towards,Elafrou2017PerformanceAA} due to its algorithmic nature, the employed compressed matrix storage format \jgl{All formats?}\christina{Yes for compressed formats (not the dense representation that includes zeros).}, and the sparsity pattern of the matrix. %\jgl{All patterns?} 
\spmv{} performs indirect memory references as a result of storing the matrix in a compressed format, and irregular memory accesses to the input vector due to sparsity. The matrices involved are very sparse, i.e., the vast majority of elements are zeros. For example, the matrices that represent Facebook’s and YouTube’s network connectivity contain 0.0003\%~\cite{YouTubeGraph,Kanellopoulos2019SMASH} and 2.31\%~\cite{FacebookGraph,Kanellopoulos2019SMASH} non-zero elements, respectively. Therefore, in processor-centric systems, \spmv{} is a bandwidth-bound kernel for the majority of sparse matrices, and is bottlenecked by data movement between memory and processors~\cite{Gomez2021Benchmarking,Elafrou2018SparseX,Elafrou2017PerformanceAA,Elafrou2019Conflict,Xie2021SpaceA}.



One promising way to alleviate the data movement bottleneck is the Processing-In-Memory (PIM)~\cite{Gomez2021Benchmarking} paradigm. PIM moves computation close to application data by equipping memory chips with processing capabilities~\cite{mutlu2020modern}. Prior works~\cite{ahn2015scalable,fernandez2020natsa,Gao2015Practical,gao2017tetris} propose PIM architectures wherein a processor logic layer is tightly integrated with DRAM memory layers using 2.5D/3D-stacking technologies. Nonetheless, the 2.5D/3D integration itself cannot provide significantly higher memory bandwidth for processors than standard DRAM~\cite{Lee2021HardwareAA,Hadi2016Chameleon}. %, because the bandwidth of each DRAM bank is often designed to match that of device I/O. 
To provide notably higher bandwidth for the processors, \textit{near-bank} PIM designs have been explored~\cite{Lee2021HardwareAA,upmem,Hadi2016Chameleon}. \textit{Near-bank} PIM designs tightly couple a PIM core with each DRAM bank, exploiting bank-level parallelism to expose high on-chip memory bandwidth of standard DRAM to processors. Moreover, manufacturers of near-bank PIM architectures avoid disturbing the key components (i.e., subarray and bank) of commodity DRAM to provide a cost-efficient and practical way for silicon materialization. Two \textit{real} near-bank PIM architectures are Samsung's FIMDRAM~\cite{Lee2021HardwareAA} and UPMEM PIM~\cite{upmem2018}.




%One promising way to alleviate the data movement bottleneck is the Processing-In-Memory (PIM)~\cite{Gomez2021Benchmarking} paradigm. PIM moves computation close to application data by equipping memory chips with processing capabilities~\cite{mutlu2020modern}. Even though several PIM architectures~\cite{Kwon2019TensorDIMM,ahn2015scalable,gao2017tetris,he2020newton,kim2016neurocube,kim2020mvid,pugsley2014ndc,yazdanbakhsh2018dram} have been explored, most of them require considerable customization of DRAM, which significantly increase the cost~\cite{Lee2021HardwareAA,Hadi2016Chameleon}, which has prevented manufacturers to commercially materialize them\jgl{Customization needs was not the reason for not manufacturing...}. However, \textit{near-bank} PIM designs place processors close to each DRAM bank, without disturbing the internal circuitry of commodity DRAM~\cite{Lee2021HardwareAA} \jgl{Not sure... So the problem was the need for modifying the DRAM array? Near-bank is easier than PuM, for sure. But what about computation in the logic layer of 3D memories? Is it more difficult to fabricate than near-bank?}. As a result, they present a cost-efficient and practical way to commercially materialize PIM architectures. Two \textit{real} near-bank PIM architectures are Samsung's FIMDRAM~\cite{Lee2021HardwareAA} and UPMEM PIM~\cite{upmem2018}.

%and constitute a cost-efficient and practical way for silicon materialization. As a result, several manufacturers have already started to commercialize 



Most near-bank PIM architectures~\cite{Hadi2016Chameleon,upmem,Lee2021HardwareAA,Gomez2021Benchmarking} support several PIM-enabled memory chips connected to a host CPU via memory channels. Each memory chip comprising multiple PIM cores, which are low-area and low-power cores with relatively low compute capabilities~\cite{Gomez2021Benchmarking}, and each of them is located close to a DRAM bank~\cite{Gomez2021Benchmarking, ke2019recnmp,Cho2020Near,Sukhan2021Hardware,upmem2018,Lee2021HardwareAA,Hadi2016Chameleon}. PIM cores can access data located on their local DRAM bank, and typically there is no direct communication channel among PIM cores. Overall, near-bank PIM architectures provide high levels of parallelism and immense memory bandwidth, thereby being very promising computing platform to accelerate memory-bound kernels. Recent works leverage near-bank PIM architectures to provide high performance and energy benefits on bioinformatics~\cite{lavenier2020Variant} and neural network kernels~\cite{Lee2021HardwareAA}. However, there is no prior work to thoroughly study the widely-used, memory-bound \spmv{} kernel on a real PIM system.
%thereby being very promising computing platform to accelerate the \spmv{} kernel. \jgl{You can mention previous works having shown successful experiences on accelerating some applications. You can also elaborate more on why SpMV is good to study (and say that noone has thoroughly studied SpMV on real PIM.}





Our work is the first to efficiently map the \spmv{} execution kernel on near-bank PIM systems, and understand its performance implications on a real PIM system. Specifically, our \textbf{goal} in this work is twofold: (i) design efficient \spmv{} algorithms to accelerate this kernel in current and future PIM systems, while covering a wide variety of sparse matrices with diverse sparsity patterns, and (ii) provide an extensive characterization analysis of the widely used \spmv{} kernel on a real PIM architecture. To this end, we provide a wide variety of \spmv{} implementations for real PIM architectures,
%present \SparseP{}~\cite{SparsePLibrary} \jgl{To achieve your goal, what you do is exploring multiple ways of implementing SpMV, not presenting SparseP...}, the first \spmv{} software package for real PIM architectures, 
and conduct a rigorous experimental analysis of \spmv{} kernels in UPMEM PIM system, the first publicly-available real-world PIM architecture.




%\jgl{Before going to the specific techniques, you should introduce the type of techniques (or implementation aspects) that you explore, and explain why you should explore them. That is, be methodical in the introduction of the techniques. What types of techniques are important for SpMV. In particular, you study: (1) load balancing within a PIM core, (2) sync within  PIM core, (3) partitioning, (4) compression formats, (5) datatypes -- modify the order as needed.}

We present \SparseP{}~\cite{SparsePLibrary} library that includes 25 \spmv{} kernels for real PIM systems, supporting various (1) data types, (2) data partitioning techniques of the sparse matrix to PIM-enabled memory, (3) compressed matrix formats, (4) load balancing schemes among PIM cores, (5) load balancing schemes among threads of a multithreaded PIM core, and (6) synchronization approaches among threads within PIM core. We support a wide range of data types, i.e., 8-bit integer, 16-bit integer, 32-bit integer, 64-bit integer, 32-bit float and 64-bit float data types to cover a variety of real-world applications that employ \spmv{} as their underlying kernel. We design two types of well-crafted data partitioning techniques: (i) the 1D partitioning technique to perform the complete \spmv{} computation only using PIM cores,
\jgl{But 2D is also "to offload the whole \spmv{} execution to PIM cores", right? In my opinion, you are going to study partitioning techniques "to offload the whole \spmv{} execution to PIM cores". Then, you will realize that 2D balances computation and data transfer better -- this can be an insight of the work. Btw, if data transfer is not needed (imaging a bigger application or a future PIM system), will 2D still be better?}\christina{I think the 1D partitioning woudl perform better in that PIM system} 
and (ii) the 2D partitioning technique to strive a balance between computation and data transfer costs to PIM-enabled memory. In the 1D partitioning technique, the matrix is horizontally partitioned across PIM cores, and the \textit{whole} input vector is copied at the DRAM bank of \textit{each} PIM core, while PIM cores directly compute the elements of the final output vector. In the 2D partitioning technique, the matrix is split in 2D tiles, the number of which is equal to the number of PIM cores, and a \textit{subset} of the elements of the input vector is copied at the DRAM bank of each PIM core. However, PIM cores create a large number of partial results for the elements of the output vector which are gathered and merged by the host CPU cores to assemble the final output vector. We support the most popular compressed matrix formats, i.e., CSR~\cite{bjorck1996numerical},  COO~\cite{Pooch1973Survey,Shubhabrata2007Scan}, BCSR~\cite{Im1999Optimizing}, BCOO~\cite{Pooch1973Survey}, and for each compressed format we implement various load balancing schemes among PIM cores to provide efficient \spmv{} execution for a wide variety of sparse matrices with diverse sparsity patterns. Finally, we design several load balancing schemes and synchronization approaches among parallel threads within a PIM core to cover real PIM systems that provide multithreaded PIM cores.


%We design two types of well-crafted data partitioning techniques: (i) an 1D partitioning technique to offload the whole \spmv{} execution to PIM cores, and (ii) a 2D partitioning technique to strive a balance between computation and data transfer costs to PIM-enabled memory \jgl{But 2D is also "to offload the whole \spmv{} execution to PIM cores", right? In my opinion, you are going to study partitioning techniques "to offload the whole \spmv{} execution to PIM cores". Then, you will realize that 2D balances computation and data transfer better -- this can be an insight of the work. Btw, if data transfer is not needed (imaging a bigger application or a future PIM system), will 2D still be better?}\christina{I think the 1D partitioning woudl perform better in that PIM system}. In the 1D partitioning technique, the matrix is horizontally partitioned across PIM cores, and the \textit{whole} input vector is copied at the DRAM bank of \textit{each} PIM core. In the 2D partitioning technique, the matrix is split in 2D tiles, the number of which is equal to the number of PIM cores, and a \textit{subset} of the elements of the input vector is copied at the DRAM bank of each PIM core. However, PIM cores create a large number of partial results for the elements of the output vector which are gathered and merged by the host CPU cores. Given that real PIM systems can include \textit{multithreaded} PIM cores to exploit immense bandwidth, \jgl{These are other types of techniques.} we implement various load balancing and synchronization approaches among multiple threads within a PIM core. \jgl{Different formats is another side of the exploration.} We support our data partitioning and load balancing schemes for the most popular compressed matrix formats, i.e., CSR~\cite{bjorck1996numerical}, COO~\cite{Pooch1973Survey,Shubhabrata2007Scan}, BCSR~\cite{Im1999Optimizing}, BCOO~\cite{Pooch1973Survey}, and a wide range of data types, i.e., 8-bit integer, 16-bit integer, 32-bit integer, 64-bit integer, 32-bit float and 64-bit double data types. 
%\jgl{I would say this at the end of the intro, right before contributions.}


%\jgl{This paragraph is a summary of results that should follow a similar structure as the previous one (after fixing the organization of the previous one).}
We conduct an extensive characterization analysis of \SparseP{} kernels on UPMEM PIM system~\cite{upmem} analyzing the \spmv{} execution using (1) one single multithreaded PIM core, (2) thousands of PIM cores, and (3) comparing it with that achieved on conventional processor-centric CPU and GPU systems. First, we characterize the limits of a single multithreaded PIM core, and show that (i) high operation imbalance among threads of a PIM core can impose high overhead in the core pipeline, and (ii) fine-grain synchronization approaches to increase parallelism cannot outperform a coarse-grain approach, if PIM hardware serializes accesses to the local DRAM memory bank. Second, we analyze the end-to-end \spmv{} execution of 1D and 2D partitioning techniques using thousand PIM cores. Our study indicates that the performance (i) of the 1D partitioning technique is limited by data transfer costs to \textit{broadcast} the whole input vector at \textit{each} DRAM bank of PIM cores, and (ii) of the 2D partitioning technique by data transfer costs to \textit{gather} partial results for the elements of the output vector from PIM-enabled memory to host CPU. Such data transfers incur high overheads, because they take place via the narrow memory bus. In addition, our detailed study across a wide variety of compressed matrix formats and sparse matrices with diverse sparsity patterns demonstrates that (i) the compressed matrix format determines the data partitioning across DRAM banks of PIM-enabled memory, thereby affecting the computation imbalance among PIM cores with the corresponding performance implications, and (ii) there is no one-size-fit all solution. The load balancing scheme among PIM cores (and among threads within PIM core) and data partitioning technique that provides the best-performing \spmv{} execution depends on the characteristics of the input matrix and the underlying PIM hardware. Finally, we compare the \spmv{} execution on UPMEM PIM system with 2528 PIM cores to state-of-the-art CPU and GPU systems, and observe that \spmv{} on UPMEM PIM achieves the closest to the peak performance. Our extensive evaluation provides programming recommendations for software designers, and suggestions and hints for hardware and system designers of future PIM systems.


%First, we characterize the limits of a single multithreaded PIM core using various load balancing and synchronization approaches among parallel threads. Our evaluations show that (i) high operation imbalance among threads of a PIM core can impose high overhead in the core pipeline, and (ii) fine-grain synchronization approaches to increase parallelism among threads cannot outperform a coarse-grain approach, if PIM hardware serializes accesses to the local DRAM memory bank. Second, we conduct a detailed evaluation of the end-to-end \spmv{} execution of 1D and 2D partitioning approaches using thousand PIM cores. Our study indicates that (i) the performance of the 1D partitioning technique is significantly limited by data transfer costs to \textit{broadcast} the whole input vector at \textit{each} DRAM bank of PIM cores, while (ii) the performance of 2D partitioning technique is highly limited by data transfer costs to \textit{gather} partial results for the elements of the output vector from DRAM banks of PIM-enabled memory to host CPU. Such data transfers incur high overheads, because they take place via the narrow expensive memory bus. In addition, we analyze various compressed matrix formats, and find that the compressed format used to store the matrix determines the data partitioning across DRAM banks of PIM-enabled memory, thereby affecting the computation imbalance among PIM cores with the corresponding performance implications. We also evaluate 26 sparse matrices with diverse sparsity patterns, and demonstrate that there is no one-size-fit all solution. The load balancing scheme among PIM cores (and among threads of a PIM core) and data partitioning technique that provides the best throughput in the \spmv{} execution depends on the characteristics of both the input sparse matrix and the underlying PIM hardware. Finally, we compare the \spmv{} execution on UPMEM PIM system with 2528 PIM cores to state-of-the-art CPU and GPU systems, and observe that \spmv{} on UPMEM PIM achieves the closest to the peak performance. Our extensive evaluation provides programming recommendations for software designers, and suggestions and hints for hardware and system designers of future PIM systems.



We highlight our most significant recommendations for software designers here:
\begin{enumerate}
    \item Design algorithms that provide high balance among threads of PIM core in terms of computations, loop control iterations, synchronization points and memory accesses.
    \item Design compressed data structures that can be effectively partitioned across DRAM banks targeting to provide high computation balance among PIM cores.
    \item Design \textit{adaptive} algorithms that both strive a balance between computation and data transfer costs, and adapt their configuration to the particular patterns of each input and the characteristics of the PIM hardware.
\end{enumerate}



We highlight our most significant suggestions for hardware and system designers here:
\begin{enumerate}
    \item Provide low-cost synchronization support and concurrent accesses to DRAM memory bank to increase parallelism on a multithreaded PIM core.
    \item Optimize the broadcast collective operation in data transfers from main memory to PIM-enabled memory to minimize overheads of copying the input data at all DRAM banks of the system.
    \item Optimize the gather collective operation \textit{at DRAM bank granularity} for data transfers from PIM-enabled memory to host CPU to minimize overheads of retrieving the output results.
    \item Design high-speed communication channels and optimized libraries for data transfers to/from hundred DRAM banks of PIM-enabled memory.
\end{enumerate}



Our \SparseP{} software package is freely and publicly available~\cite{SparsePLibrary} to enable further research on \spmv{} in current and future PIM systems. To sum up, the main contributions of this work are as follows:
\begin{itemize}
    \item We present \SparseP{}, the first open-source \spmv{} software package for real PIM architectures. \SparseP{} includes 25 \spmv{} kernels, supporting the four most widely used compressed matrix formats and a wide range of data types. \SparseP{} is publicly available, and can be useful for researchers to improve multiple aspects of future PIM hardware and software. 
    \item We perform the first comprehensive study of the widely used \spmv{} on UPMEM PIM architecture, the first real PIM architecture. We analyze performance implications of \spmv{} PIM execution using a wide variety of (1) compressed matrix formats, (2) data types, (3) data partitioning and load balancing techniques, and (4) 26 matrices with diverse sparsity patterns.
    \item We compare the performance and energy of \spmv{} on UPMEM PIM system with 2528 PIM cores, i.e., the first publicly-available real-world PIM architecture, to state-of-the-art CPU and GPU systems. The \spmv{} achieves less than 1\% of the peak performance on processor-centric CPU and GPU systems, while it achieves on average 51.7\% of the peak performance on UPMEM PIM system, thus highly leveraging the computation capabilities of underlying hardware. UPMEM PIM system can also provide high-energy efficiency on the \spmv{} kernel.
\end{itemize}


 








==> backup/backup1/2-background.tex <==

\section{Real PIM Architecture}\label{sec:upmem_pim}
\jgl{I would have a single background section that starts with SpMV and compression formats. Then, show SpMV is memory bound and suggest PIM as the solution. Then, introduce PIM with a near-bank PnM generic design, which is common to FIMDRAM, UPMEM, etc. Then, give a few more details about UPMEM.}

This section describes the baseline near-bank PIM architecture, and UPMEM PIM system.

\subsection{Baseline Near-bank PIM Architecture}
\jgl{Check the recent PIM theoretical model paper in SPAA. Their generic architecture looks more generic than this one, but it is applicable here too.}
Numerous works~\cite{ke2019recnmp,Lee2021HardwareAA,upmem2018,Gomez2021Benchmarking,Hadi2016Chameleon,li2017drisa,tensordimm,li2018scope,huangfu2019medal,ke2021near} show the potential benefits of near-bank PIM architectures for irregular applications. Figure~\ref{fig:near-bank-pim} shows the baseline organization of a PIM system that we assume in this work. The PIM system (Figure~\ref{fig:near-bank-pim} left) consists of a host CPU, standard DRAM memory modules, and PIM-enabled memory modules. PIM-enabled modules are connected using one or more memory channels, and include multiple PIM chips. A PIM chip (Figure~\ref{fig:near-bank-pim} right) includes a low-area PIM core with small private instruction and data memories, and a DRAM bank. PIM cores can access data located on their local DRAM bank, and typically there is no direct communication channel among PIM cores. The DRAM banks of PIM chips are accessible by the host CPU for copying input data and retrieving results via the memory bus.


\begin{figure*}[h]
    \vspace{-8pt}
    \centering
    \includegraphics[width=0.99\linewidth]{background/PIM-system.pdf}
    \vspace{-4mm}
    \caption{High-level organization of an near-bank PIM architecture.}
    \label{fig:near-bank-pim}
    \vspace{-10pt}
\end{figure*}


\subsection{UPMEM PIM Architecture}
The UPMEM PIM system includes the host CPU with standard main memory, and UPMEM modules. An UPMEM module is a standard DDR4-2400 DIMM with 2 ranks. Each rank contains 64 PIM cores, which are called \underline{D}RAM \underline{P}rocessing \underline{U}nits (DPUs). In current UPMEM PIM system, there are 20 double-rank PIM DIMMs with 2560 DPUs.\footnote{There are thirty two faulty DPUs in the system where we run our experiments. They cannot be used and do not affect the correctness of our results, but take away from the system’s full computational power of 2560 DPUs.}


\noindent\textbf{DPU Architecture and Interface.} Each DPU has exclusive access to a 24-KB instruction memory, named \textbf{IRAM}, a 64-KB scratchpad memory, named \textbf{WRAM}, and 64-MB DRAM bank, named \textbf{MRAM}. A DPU is a multithreaded in-order 32-bit RISC core that runs at 350MHz \jgl{The new one is faster.}. The DPU has 24 hardware threads, each of them has 24 32-bit general purpose registers. The DPU pipeline has 14 stages, and supports a single cycle 8x8-bit multiplier. Multiplications on 64-byte integers, floats, doubles are not supported in hardware, and require longer routines with a high number of operations~\cite{Gomez2021Benchmarking,upmem}. Threads share the IRAM and WRAM, and can access the MRAM by executing transactions in 64-bit granularity via a DMA engine, i.e., data can be accessed from/to MRAM as a multiple of 8 bytes, up to 2048 bytes. MRAM transactions are serialized in the DMA engine. The ISA provides DMA instructions to move instructions from MRAM to IRAM, or data between MRAM and WRAM. The DPU access the WRAM through 8-, 16-, 32- and 64-bit load/store instructions. DPUs use the \textit{Single Program Multiple Data} programming model, where software threads, called \textbf{tasklets}, execute the same code, but operate in different pieces of data, and can execute different control-flow paths during runtime. Tasklets can synchronize using mutexes, barriers, handshakes and semaphores provided by UPMEM runtime library.


\noindent\textbf{CPU-DPU Data Transfers.} Standard main memory and PIM-enabled memory have different data layouts. Main memory uses the conventional horizontal mapping~\cite{devaux2019,Vivek2015Gather}, which maps consecutive 8-bit words onto consecutive DRAM chips. PIM-enabled memory maps 64-bit words in the same MRAM bank~\cite{devaux2019}. The UPMEM SDK has a transposition library to execute necessary data shuffling when moving data between main memory and MRAM banks. The data transformations are programmer-transparent. The CPU-DPU and DPU-CPU data transfers can be performed in parallel, i.e., concurrently across multiple MRAM banks, requiring \textit{the transfer sizes from/to all MRAM banks be the same}. The UPMEM SDK provides two options: (i) perform parallel transfers to all MRAM banks of all ranks, and (ii) iterate over each rank to perform parallel transfers to MRAM banks of the same rank, and serialize data transfers across ranks.

\jgl{I wonder how much of the information here included is really necessary to understand the rest of the paper. For sure, readers do not need to know that there is a transposition library...}


\section{Sparse Matrix Vector Multiplication}

\jgl{SpMV is the center of the paper. We should talk about it early in the background. Several things that I would like to see in this section are: (1) a formal description of SpMV and/or a pseudocode, (2) a more comprehensive subsection about compression formats where also other formats are mentioned (e.g., CSC, bitmap-based, ELL, JDS...), and you justify why the 4 chosen ones, (3) a characterization of SpMV on CPU/GPU (or at least enough references and discussion) about memory boundedness and the need for reducing data movement -- btw, that analysis of the fraction of peak throughput fits in here, among other ways of characterizing.}

The \spmv{} kernel multiples a matrix of size $mxn$ with an input vector of size $1xn$ to compute the output vector of size $mx1$. Since matrices involved are highly sparse~\cite{Kanellopoulos2019SMASH,Elafrou2018SparseX,Elafrou2017PerformanceAA}, they are stored in a compressed format. We describe 
the most widely used compressed formats (Figure~\ref{fig:sparse_formats}).




\begin{figure*}[h]
    \vspace{-8pt}
    \centering
    \includegraphics[width=0.99\linewidth]{background/Sparse_Formats.pdf}
    \vspace{-10pt}
    \caption{(a) \spmv{} with a dense matrix representation, and (b) CSR, (c) COO, (d) BCSR, (e) BCOO formats. \jgl{BCSR and BCOO are not clear. Btw, fix the labels.}}
    \label{fig:sparse_formats}
    \vspace{-10pt}
\end{figure*}


\noindent\textbf{Compressed Sparse Row (CSR)~\cite{bjorck1996numerical}.} The CSR format (Figure~\ref{fig:sparse_formats}b) sequentially stores values in row order. An array, named rowptr[], stores the index pointers that represent the number of non-zero elements of each row. The adjacent pair rowptr[i], rowptr[i+1], stores the index of the non-zero element that start and stop for the i-th row. A column index array (colind[]) and a value array (values[]), store the column index and value of each non-zero element, respectively.


\noindent\textbf{Coordinate Format (COO)~\cite{Pooch1973Survey,Shubhabrata2007Scan}.} The COO format (Figure~\ref{fig:sparse_formats}c) stores the non-zero elements as a series of tuples (tuples[] array). Each tuple includes the row index, column index, and value of the non-zero element. 



\noindent\textbf{Block Compressed Sparse Row (BCSR)~\cite{Im1999Optimizing}.} The BCSR format (Figure~\ref{fig:sparse_formats}d) is a block representation of CSR. The browptr[] stores the index pointers that represent the number of non-zero blocks of each block row \jgl{What is a block row?}, and the bcolind[] store the column index of a non-zero block within a block row. The bvalues[] array is a dense representation of the values of the non-zero blocks. Figure~\ref{fig:sparse_formats}d shows an example of BCSR for block sizes of 4×4.





\noindent\textbf{Block Coordinate Format (BCOO)~\cite{Pooch1973Survey}.} The BCOO format is the block counterpart of COO. The browind[], bcolind[] and  bvalues[] arrays store the row indices, column indices and values of the non-zero blocks, respectively. Figure~\ref{fig:sparse_formats}e shows a BCOO example for block sizes of 4×4.








==> backup/backup1/3-SparseP.tex <==
\section{\SparseP{} Library}
\jgl{To me, this paper is not about presenting a library. That is just a byproduct of the work. The interesting contribution of the work is the exploration of all techniques. For that reason, I would have an overview section that introduces and justifies all techniques that are explored in the work. After that, you can have different sections elaborating on the different techniques.}
%\jgl{I would start with the techniques that are relevant inside a single PIM core (i.e., load balancing, sync). Then, go for partitioning across PIM cores in the next section.} % JGL: I commented this out.

This section presents the \spmv{} kernels of \SparseP{} package. Section~\ref{sec:lib_kernel} describes the \spmv{} execution in a PIM system. Section~\ref{sec:lib_1d-2d} and Section~\ref{sec:lib_1dpu} describe parallelization techniques among PIM cores, and among threads within a PIM core, respectively.


\subsection{The \spmv{} execution in a PIM system}\label{sec:lib_kernel}
Figure~\ref{fig:spmv-pim-execution} shows the \spmv{} execution in a PIM system, which is broken down in four steps: (1) the time to load the input vector at DRAM banks of PIM-enabled memory (\textbf{load}), (2) the kernel time to execute \spmv{} on PIM cores (\textbf{kernel}), (3) the time to retrieve from DRAM banks to the host CPU results for the output vector (\textbf{retrieve}), and (4) the time to merge partial results and assemble the final output vector on the host CPU (\textbf{merge}). In our analysis, we omit the time to load the matrix at PIM-enabled memory, since this step can be typically hidden in real-world applications (it can be overlapped with other computation performed by the application or amortized if the application performs multiple \spmv{} iterations on the same matrix). \jgl{Can't the load time of the input vector be overlapped too? I have the feeling that we put too much emphasis on the transfers.} \jgl{Btw, retrieving the results (3) can also be overlapped with the merging of partial results (4). Do we do that?}



\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{partitioning_figures/SPMV_PIM_execution.pdf}
    \vspace{-4mm}
    \caption{The execution of the \spmv{} kernel in a real PIM system.}
    \label{fig:spmv-pim-execution}
\end{figure}


\noindent\textbf{Kernel Implementation.}
We briefly describe the \SparseP{} kernel implementations for all compressed matrix formats, i.e., the way that threads access data involved in the kernel from/to the local DRAM bank. The \spmv{} kernels includes three types of data structures: (i) the arrays that store the non-zero elements, i.e., the values (values[] \jgl{Use Courier font for these.}) and the positions of the non-zero elements (e.g., rowptr[], colind[] for CSR format, tuples[] for COO format, browptr[], bcolind[] for BCSR format, browind[], bcolind[] for BCOO format), (ii) the array that stores the values of the elements of the input vector, and (iii) the array that stores the partial results created during \spmv{} PIM execution for the elements of the output vector. First, the arrays that store the non-zero elements are compressed data structures that accessed in a streaming way. Thus, to exploit spatial locality and immense bandwidth, each thread reads the non-zero elements of the matrix by fetching large chunks of these arrays in a coarse-gran manner from DRAM memory to data (scratchpad) memory, and then accesses elements through data (scratchpad) memory in a fine-grain manner. In UPMEM PIM system, we fetch chunks of 256-byte data from MRAM to WRAM, as suggested by prior work~\cite{Gomez2021Benchmarking}, since 256 bytes transfer sizes fully exploit the available local bandwidth of MRAM \jgl{Why 256 bytes? The bandwidth is maximum with 1024-2048 bytes}. In BCSR and BCOO formats, we fetch the values of the non-zero elements (bvalues[] array) from DRAM to data (scratchpad) memory in chunks equal to the bytes of 2D block size (e.g., 4x4 elements) used. Second, the elements of the input vector are accessed with an irregular way, i.e., the accesses are neither streaming nor strided, while they are input-driven, since they are determined by the column positions of the non-zero elements of each particular matrix. In CSR and COO formats, given that there is neither spatial and temporal locality in the array of the input vector, threads of a PIM core directly access elements of the input vector through DRAM memory arrays in fine-granularity~\cite{Gomez2021Benchmarking,upmem-guide}, i.e., using the smallest possible granularity, which in UPMEM PIM system is 64-bits. In BCSR and BCOO formats, threads fetch elements of the input vector from DRAM to data (scratchpad) memory in chunks of equal to the bytes of one dimension of the block size used. Finally, during \spmv{} execution, threads sequentially traverse non-zero elements at row order for CSR and COO formats and at block-row order for BCSR and BCOO formats. Thus, threads produce partial results based on the non-zero elements of the \textit{same} row for CSR and COO formats and of the \textit{same} block row for BCSR and BCOO formats. Threads temporarily store results for elements of the output vector in data (scratchpad) memory to exploit data locality. Then, the produced results are written in DRAM memory with a fine-granularity~\cite{Gomez2021Benchmarking,upmem-guide} (e.g., 64-bits in UPMEM PIM architecture) for CSR and COO formats, and with a granularity equal to the dimension of the block size used in BCSR and BCOO formats. Note that in COO and BCOO formats, the output vector needs to be initialized with zero values before the execution of the main \spmv{} kernel. In this case, threads perform bulk write accesses to DRAM in a coarse-grain manner, e.g., 256-byte granularity in UPMEM PIM architecture~\cite{Gomez2021Benchmarking,upmem-guide}.
\jgl{This whole paragraph is too difficult to follow. You need to be more methodical in the explanation. You need figures or pseudocodes to illustrate too. Btw, you talk about the kernel here, then about the partitioning across DPUs, then optimizations for the kernel... The flow does not make sense to me. Either start from the top or from the bottom, but do not go back and forth.}


%write accesses on the output vector typically exhibit a non-fixed stride pattern due to high sparsity of the matrix. Thus, hardware threads write partial results of the output vector through DRAM in fine-granularity~\cite{Gomez2021Benchmarking} (64-bits in UPMEM PIM architecture). 

%The arrays that store the non-zero elements (i.e., values[]), and their positions (i.e., rowptr[], colind[] for CSR, tuples[] for COO, browptr[], bcolind[] for BCSR, browind[], bcolind[] for BCOO) are accessed in streaming way. To exploit spatial locality and immense bandwidth, we fetch chunks of elements for these arrays in a coarse-grain manner from DRAM to data (scratchpad) memory, and access elements through data memory in a fine-grain manner. The elements of the input vector are accessed with an irregular way, i.e., the accesses in the input vector are neither streaming nor strided, while they are input-driven, since they are determined by the column positions of the non-zero elements of each particular matrix. Thus, we directly access elements of the input vector through DRAM in fine-granularity~\cite{Gomez2021Benchmarking,upmem-guide}, i.e., using the smallest possible granularity (64-bits in UPMEM PIM architecture). Finally, the accesses on the elements of the output vector can be strided, however with a non-fixed stride pattern, thus we write elements of the output vector through DRAM in fine-granularity, as suggested in prior work~\cite{Gomez2021Benchmarking,upmem-guide}. When the elements of the output vector need to be initialized with zeroes (e.g., COO/BCOO formats), we perform bulk DRAM writes in a coarse-grain manner.



\subsection{Parallelization Techniques Among PIM Cores}\label{sec:lib_1d-2d}
To parallelize the \spmv{} kernel, we implement well-crafted data partitioning schemes across multiple DRAM banks. In \SparseP{}, matrices are stored in a row-sorted way, i.e., the non-zero elements are sorted in increasing order on their row indices. Specifically, each PIM core computes results for a \textit{continuous} subset of elements of the output vector. This way we avoid transferring to the host CPU a list with the indices of the elements for the output vector which were produced at each particular PIM core, and thus we avoid additional data transfer overheads. \SparseP{} supports two types \jgl{I can see four.} of partitioning techniques, shown in Figure~\ref{fig:partitioning}. 
\jgl{Would there be any benefit from not assigning continuous elements? If no benefit (regardless of the data transfer overhead), no need to mention it -- it would be obvious.}


\begin{figure}[H]
    \centering
    \includegraphics[width=1\textwidth]{partitioning_figures/Partitioning_techniques5.pdf}
    \vspace{-12pt}
    \caption{The \SparseP{} partitioning techniques assuming 4 PIM cores and 2 vertical partitions for the 2D partitioning schemes.}
    \label{fig:partitioning}
\end{figure}


\jgl{Why don't we have 1D of variable size? I think it is a fair question. It would be good to avoid it by providing proper justification.}
First, we provide an 1D partitioning technique (Figure~\ref{fig:partitioning}a), in which the matrix is horizontally partitioned across PIM cores, and the whole input vector is copied at the DRAM bank of each core. With the 1D partitioning technique, the \spmv{} execution is completely offloaded to PIM cores, since the merge step in the host CPU is negligible: a very small number of partial results are created, i.e., only for a few rows which are split across neighboring PIM cores. Thus, the number of partial elements of the output vector is at most equal to the number of PIM cores used. Second, we provide 2D partitioning techniques (Figure~\ref{fig:partitioning}b-d), in which the matrix is partitioned in 2D tiles, the number of which is equal to the number of PIM cores. With the 2D partitioning technique, we aim to strive a balance between computation and data transfer costs, since a subset of the elements of the input vector is copied at the DRAM bank of each PIM core. However, PIM cores assigned to horizontally overlapped tiles \jgl{Clarify the meaning} produce many partial results for the elements of the output vector. These partial results are transferred to the host CPU, and merged by CPU cores, which assemble the final output vector. In \SparseP{} library, the \textit{merge} step performed by the CPU cores is parallelized using the OpenMP API~\cite{Dagum98OpenMP}.



\SparseP{} includes three 2D partitioning techniques:
\begin{enumerate}
    \item \textbf{\equallySized} (Figure~\ref{fig:partitioning}b): The 2D tiles are statically created to have the same height and width. This way the subsets of the elements for the input and output vectors have the same sizes among all PIM cores.
    \item \textbf{\equallyWidth} (Figure~\ref{fig:partitioning}c): The 2D tiles have the same width and variable height. This way the subset of the elements for the input vector has the same size among PIM cores, while the subset of the elements for the output vector varies among PIM cores. We balance the non-zero elements among the tiles of the \textit{same} vertical partition, such that provide high non-zero balance among PIM cores assigned to the same vertical partition.
    \item \textbf{\variableSized} (Figure~\ref{fig:partitioning}d): The 2D tiles have both variable width and height. We balance the non-zero elements both among the vertical partitions and among the tiles of the \textit{same} vertical partition. This way we \juan{can} provide high-non zero balance among all PIM cores.
\end{enumerate}



\begin{table}[b]
\vspace{-2pt}
\centering
\begin{minipage}{0.49\linewidth}
%\ra{0.9}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{| l | l | l | l |} 
 \toprule
 Partitioning & Compressed & Load Balancing  \\ 
 Technique & Format & Among PIM Cores  \\ [0.5ex] \midrule \midrule
% \hline\hline
    \multirow{9}{*}{\hspace*{2.1em}\turnbox{0}{1D}} & \multirow{2}{*}{CSR} &  rows (\textbf{CSR.row})  \\
    & & nnz$^{\star}$ (\textbf{CSR.nnz}) \\ \cline{2-3}
    & \multirow{2}{*}{COO} &  rows (\textbf{COO.row}) \\
    & & nnz$^{\star}$ (\textbf{COO.nnz-rgrn})  \\
    & & nnz (\textbf{COO.nnz}) \\  \cline{2-3}
    & \multirow{2}{*}{BCSR} &  blocks$^{\dagger}$ (\textbf{BCSR.block})   \\
    & & nnz$^{\dagger}$ (\textbf{BCSR.nnz}) \\  \cline{2-3}
    & \multirow{2}{*}{BCOO} &  blocks (\textbf{BCOO.block}) \\
    & & nnz (\textbf{BCOO.nnz}) \\ \hline
    \multirow{4}{*}{\shortstack{2D \\ \equallySized}} & CSR (\textbf{dcsr}) & - \\  \cline{2-3}
    &  COO (\textbf{dcoo}) & -  \\  \cline{2-3}
    &  BCSR (\textbf{dbcsr}) & -  \\  \cline{2-3}
    &  BCOO (\textbf{dbcoo}) & - \\ \hline
 \bottomrule
\end{tabular}
}
\end{minipage} \hspace{1pt}%
\begin{minipage}{0.49\linewidth}
%\ra{0.9}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{| l | l | l | l |} 
 \toprule
 Partitioning & Compressed & Load Balancing  \\ 
 Technique & Format & Among PIM Cores  \\ [0.5ex] \midrule \midrule
% \hline\hline
  \multirow{6}{*}{\shortstack{2D \\ \equallyWidth}} &  CSR (\textbf{rbdcsr}) & nnz$^{\star}$ \\  \cline{2-3}
    &  COO (\textbf{rbdcoo}) & nnz  \\  \cline{2-3}
    & \multirow{2}{*}{BCSR} & blocks$^{\dagger}$ (\textbf{rbdbcsr}) \\
    &  & nnz$^{\dagger}$ \\ \cline{2-3}
    & \multirow{2}{*}{BCOO} & blocks (\textbf{rbdbcoo})  \\ 
    & & nnz  \\ \hline     
  \multirow{6}{*}{\shortstack{2D \\ \variableSized}} &  CSR (\textbf{bdcsr}) & nnz$^{\star}$  \\ \cline{2-3}
    &  COO (\textbf{bdcoo}) & nnz   \\  \cline{2-3}
    &  \multirow{2}{*}{BCSR} & blocks$^{\dagger}$ (\textbf{bdbcsr})  \\
    &  & nnz$^{\dagger}$ \\ \cline{2-3}
    &  \multirow{2}{*}{BCOO } & blocks (\textbf{bdbcoo}) \\ 
    &  &  nnz  \\      
 \bottomrule
\end{tabular}
}
\end{minipage} \hspace{1pt}% 
\vspace{-1pt}
\caption{Pallelization techniques among PIM cores of \SparseP{}. $^{\star}$: row-granularity, $^{\dagger}$: block-row-granularity}
\label{table:library}
\vspace{-10pt}
\end{table}


Table~\ref{table:library} shows the parallelization approaches among PIM cores. Please also see Appendix~\ref{sec:appendix-sparseP} for all \spmv{} kernels provided by \SparseP{} software package.  All kernels support a wide range of data types, i.e., 8-bit integer (\textbf{int8}), 16-bit integer (\textbf{int16}), 32-bit integer (\textbf{int32}), 64-bit integer (\textbf{int64}), 32-bit float (\textbf{flt32}), and 64-bit double (\textbf{dbl64}) data types. \jgl{Table 1 should go here.}


\subsubsection{\textbf{Load Balancing Approaches in the 1D Partitioning.}} \SparseP{} provides various load balancing schemes among PIM cores. For CSR and COO formats, we balance either the rows, such that each PIM core processes almost the same number of rows, or the non-zero elements, such that each PIM core processes almost the same number of non-zero elements. In CSR format, the matrix is stored in row-order, thus balancing the non-zero elements is performed at a row granularity. %\SparseP{} provides a row-sorted COO implementation, i.e., tuples are stored in increasing order on their row indices, such that each PIM core computes results for \textit{continuous elements} of the output vector. This way we avoid transferring to the host CPU a list with the indices of the elements for the output vector, which were produced at each particular PIM core, and thus we avoid additional data transfer overheads. 
In COO format, balancing the non-zero elements can be performed either in a row granularity, or by splitting a row across two neighboring PIM cores to provide a perfect non-zero element balance among cores. In the later case, as explained, a small number of partial results is merged by the host CPU: between two neighboring PIM cores at most one element might need to be accumulated at the host CPU cores.
\jgl{Indeed there are two ways of 1D partitioning. You should describe them generically and then explain the particularities for each compression format. And then particularities due to UPMEM architecture (I mean, there might be implementation decisions that are inherent to the format and others forced by the specific PIM architecture.}



For BCSR and BCOO formats, we balance either the blocks, such that each PIM core processes almost the same number of blocks, or the non-zero elements, such that each PIM core processes almost the same number of non-zero elements. In BCSR format, the matrix is stored in block-row order, thus balancing the non-zero elements among cores is performed in a block-row granularity. %\SparseP{} provides a block-row-sorted BCOO implementation, i.e., the matrix is stored in increasing order on block-row indices, such that each PIM core computes results for \textit{continuous elements} of the output vector to improve performance. 
In BCOO format, given that a block-row might be split across two PIM cores, a small number of partial results is merged by the host CPU: between two neighboring PIM cores at most block size elements of the output vector might need to be accumulated at the host CPU.





\subsubsection{\textbf{Load Balancing Approaches in the 2D Partitioning.}} \SparseP{} provides various load balancing schemes among PIM cores in the \equallyWidth{} and \variableSized{} techniques. In the \equallyWidth{} technique, for CSR and COO formats, we balance the non-zero elements among the tiles of the same vertical partition. The load balancing in the CSR format is performed in a row-granularity \jgl{Meaning?}. For BCSR and BCOO formats, we balance either the blocks or the non-zero elements among the tiles of the same vertical partition. The load balancing in the BCSR format is performed in a block-row granularity \jgl{Meaning?}. In the \variableSized{} technique, we first balance the non-zero elements among the vertical partitions, such that the vertical partitions include the same number of non-zero elements. Then, among the tiles of the same vertical partition, we balance the non-zero elements for CSR (in a row-granularity) and COO formats, and either the blocks or the non-zero elements for BCSR (in a block-row granularity) and BCOO formats.

\jgl{These explanations would greatly benefit from figures illustrating toy examples.}


\subsection{Parallelization Techniques Among Threads within a PIM Core}\label{sec:lib_1dpu}
PIM cores can support multiple hardware threads to exploit immense bandwidth. Therefore, \SparseP{} supports various load balancing approaches for each compressed matrix format, and three synchronization approaches to ensure correctness among threads of a PIM core.





\subsubsection{\textbf{Load Balancing Approaches.}}
For CSR and COO formats, we balance either the rows, such that each thread processes almost the same number of rows, or the non-zero elements, such that each thread processes almost the same number of non-zero elements \jgl{Observe how this is the same as across PIM cores. It is possible to start explaining things at a higher level, and then go to the details across PIM cores / inside a PIM core}. In CSR format, matrix is stored in row-order, thus load balancing among threads is performed in a row granularity. In UPMEM PIM system, elements of the output vector are accessed in 64-bit granularity in DRAM. Thus, when balancing is performed in a row granularity, we assign rows to threads in chunks of $8 / sizeof(data\_type)$ to ensure 8-byte alignment on the elements of the output vector. In COO format, balancing the non-zero elements can be performed either in a row-granularity or by splitting the row, i.e., providing an almost perfect non-zero balance among threads. In the latter case, synchronization among threads for writes on the elements of the output vector can be implemented with the three synchronization approaches described in the next section. \jgl{Again, note that this is the same across PIM cores: you need to synchronize in some way. Across PIM cores there is only a way to do it in the UPMEM system (via host), but we could think about a cross-PIM-core network and sync primitives -- this is an opportunity to cite SynCron and give recommendations.}



For BCSR and BCOO formats, we balance either the blocks, such that each thread processes almost the same number of blocks, or the non-zero elements, such that each thread processes almost the same number of non-zero elements. In BCSR format, the matrix is stored in block-row order, thus load balancing among threads is performed in a block-row granularity. For both formats, the block sizes are \textit{configurable} in \SparseP{}. In our evaluation, we use block sizes of 4x4 \jgl{Did we do no sensitivity analysis?}, similarly to prior work~\cite{asgari2020copernicus} \jgl{This is very much an architecture-dependent decision...}. In UPMEM PIM architecture, elements of the output vector are accessed in 64-bit granularity. Therefore, in case of 4x4 block sizes and 8-bit integer for BCSR format, we include synchronization primitives in the output vector, since different threads may write on the same 64-bit aligned DRAM location. Synchronization among threads for writes on the elements of the output vector can be implemented with the approaches described next.






\subsubsection{\textbf{Synchronization Approaches.}}
\SparseP{} provides three synchronization approaches.
\begin{enumerate}
\item \textbf{Coarse-grain Locking (\textcolor{darkred}{lb-cg}).} One global mutex protects the elements of the whole output vector.
\item\textbf{Fine-grain Locking (\textcolor{darkred}{lb-fg}).} Multiple mutexes protect the elements of the output vector. \SparseP{} associates mutexes to the elements of the output vector in a round-robin manner. The UPMEM API supports up to 56 mutexes. In our evaluation, we use 32 mutexes such that to find the corresponding mutex for a particular element of the output vector only with shift operation on the MRAM address, and avoid costly division operations.
\item\textbf{Lock-free (\textcolor{darkred}{lf}).} Since the formats are row-sorted for CSR/COO and block-row sorted for BCSR/BCOO, race conditions in the output vector arise \textit{only in a few elements}, i.e., either when a row (or a block row for BCSR/BCOO) is split across threads, or in UPMEM PIM system, when continuous elements of the output vector processed by different threads belong to the same 64-bit aligned MRAM location. In our lock-free approach, threads temporarily store partial results for these few elements in the data (scratchpad) memory, and later one single thread merges the partial results, and writes the final result for the corresponding element of the output vector to DRAM memory bank.
\jgl{I'm not sure about calling this "lock-free". To me, lock free uses CAS operations. Anyway, a barrier (a way of locking) is needed after all threads write in the scratchpad.}

\jgl{In the end, these are just different ways of implementing a reduction operation. There is also a reduction in the host.}
\end{enumerate}




Table~\ref{table:1DPU-impl} summarizes the parallelization techniques among threads of a PIM core. All kernels support a wide range of data types, i.e., 8-bit integer (\textbf{int8}), 16-bit integer (\textbf{int16}), 32-bit integer (\textbf{int32}), 64-bit integer (\textbf{int64}), 32-bit float (\textbf{flt32}), and 64-bit double (\textbf{dbl64}) data types. \jgl{Are flt32 and dbl64 common abbreviations? I'd prefer fp32 and fp64.}






\begin{table}[H]
\vspace{-2pt}
\centering
%\ra{0.9}
\begin{minipage}{0.68\linewidth}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{| l | l | l |} 
 \toprule
  Compressed & Load Balancing & Synchronization  \\ 
  Format & Among Threads & Approach  \\
  [0.5ex] \midrule \midrule
% \hline\hline
   \multirow{2}{*}{CSR} & rows (\textbf{CSR.row}) & -  \\
   & nnz$^{\star}$ (\textbf{CSR.nnz}) & -   \\ \hline
   \multirow{3}{*}{COO} & rows (\textbf{COO.row}) & -   \\
   & nnz$^{\star}$ (\textbf{COO.nnz-rgrn}) & -   \\
   & nnz (\textbf{COO.nnz}) & lb-cg / lb-fg / lf   \\ \hline
   \multirow{2}{*}{BCSR} & blocks$^{\dagger}$ (\textbf{BCSR.block}) & lb-cg / lb-fg (only for int8 and 4x4 block sizes)   \\
   & nnz$^{\dagger}$ (\textbf{BCSR.nnz}) & lb-cg / lb-fg (only for int8 and 4x4 block sizes)  \\  \hline
   \multirow{2}{*}{BCOO} & blocks (\textbf{BCOO.block}) & lb-cg / lb-fg / lf \\
   & nnz (\textbf{BCOO.nnz}) & lb-cg / lb-fg / lf  \\
 \bottomrule
\end{tabular}
}
\end{minipage}
\caption{Parallelization schemes among threads of a PIM core. 
$^{\star}$: row-granularity, $^{\dagger}$: block-row-granularity \jgl{"(only for int8...)" -- is this explained anywhere?}}
\label{table:1DPU-impl}
\end{table}


==> backup/backup1/4-1DPU.tex <==

%\section{Performance Characterization of One DPU}
\section{Analysis of \spmv{} Execution on One DPU}\label{1DPU}

\jgl{We should have a methodology section that talks about the system, the matrices for the different experiments, etc.}


This section analyzes the \spmv{} execution using a single DPU in UPMEM PIM architecture. In all our experiments presented henceforth, we use an UPMEM PIM system that includes a 2-socket Intel Xeon Silver 4110 CPU at 2.10GHz as the host CPU, standard main memory (DDR4-2400) of 128GB, and 20 UPMEM PIM DIMMs with 160GB PIM-capable memory. Table~\ref{tab:small-matrices} shows our evaluated small matrices that fit at 64MB of a single DPU. The evaluated matrices vary in sparsity (i.e., NNZ / (rows x columns)), standard deviation of non-zero elements among rows (NNZ-r-std) and columns (NNZ-c-std). The highlighted matrices in Table~\ref{tab:small-matrices} with red color exhibit block pattern~\cite{Kourtis2011CSX,Elafrou2018SparseX}.





\begin{table}[H]
\begin{center}
\centering
\begin{minipage}{.48\linewidth}
%\resizebox{1.0\linewidth}{0.13\textheight}{
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|l|r|r|r|}
    \toprule
    \textbf{Matrix Name} & \textbf{Sparsity} & \textbf{NNZ-r-std} & \textbf{NNZ-c-std} \\
    \midrule
    delaunay\_n13  & 	7.32e-04 &  1.343  & 1.343 \\ \hline 
    wing\_nodal &	1.26e-03 &  2.861 & 2.861 \\ 
    \bottomrule
\end{tabular}
}
\end{minipage} % 
\begin{minipage}{.48\linewidth}
%\resizebox{1.0\linewidth}{0.13\textheight}{
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|l|c|r|r|r|r|}
    \toprule
    \textbf{Matrix Name} & \textbf{Sparsity} & \textbf{NNZ-r-std} & \textbf{NNZ-c-std} \\
    \midrule
    \textcolor{darkred}{raefsky4} & 3.396e-03  & 15.956 & 15.956 \\ \hline 
    \textcolor{darkred}{pkustk08} & 0.006542 &  61.537 &  61.537 \\     
    \bottomrule
\end{tabular}
}
\end{minipage} 
\end{center}
\vspace{-2pt}
\caption{Small Matrix Dataset.}
\label{tab:small-matrices}
\end{table}





%\subsection{\textbf{Load Balancing Techniques Among Tasklets of One DPU}}\label{1DPU-MulTskl}
\noindent{\textbf{Load Balancing Techniques Among Tasklets of A Single DPU.}} Figure~\ref{fig:1DPU-datatypes} compares the load balancing schemes of various compressed matrix formats, presented in Table~\ref{table:1DPU-impl}, using 16 tasklets of one single DPU \jgl{Why 16? Don't we analyze by number of tasklets first?}. For BCSR and BCOO formats, we omit results for the fine-grain locking approach, since it performs similarly with the coarse-grain locking approach, as we demonstrate in Appendix ~\ref{sec:appendix-1DPU-BCOO} \jgl{Still it is necessary to explain here why they perform similarly}.





\begin{figure}[t]
\centering
\begin{minipage}{\textwidth}
\includegraphics[width=.245\textwidth]{1DPU/csr_datatypes_delaunay-n13_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/csr_datatypes_wing-nodal_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/csr_datatypes_raefsky4_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/csr_datatypes_pkustk08_16.pdf}
\end{minipage}\hspace{2pt}%
\begin{minipage}{\textwidth}
\includegraphics[width=.245\textwidth]{1DPU/coo_datatypes_delaunay-n13_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/coo_datatypes_wing-nodal_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/coo_datatypes_raefsky4_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/coo_datatypes_pkustk08_16.pdf}
\end{minipage}\hspace{2pt}%
\begin{minipage}{\textwidth}
\includegraphics[width=.245\textwidth]{1DPU/bcsr_datatypes_delaunay-n13_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/bcsr_datatypes_wing-nodal_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/bcsr_datatypes_raefsky4_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/bcsr_datatypes_pkustk08_16.pdf}
\end{minipage}\hspace{2pt}%
\begin{minipage}{\textwidth}
\includegraphics[width=.245\textwidth]{1DPU/bcoo_datatypes_delaunay-n13_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/bcoo_datatypes_wing-nodal_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/bcoo_datatypes_raefsky4_16.pdf}
\includegraphics[width=.245\textwidth]{1DPU/bcoo_datatypes_pkustk08_16.pdf}
\end{minipage}
\vspace{-8pt}
\caption{Execution time achieved by 16 tasklets of a single DPU for various load balancing schemes.}
\label{fig:1DPU-datatypes}
\end{figure}


We draw out four findings \juan{from Figure~\ref{fig:1DPU-datatypes}}. First, we find that the \spmv{} executions using int8, int16, and int32 data types achieve similar execution time among them, since the multiplication operation of these data types is sufficiently supported by hardware~\cite{Gomez2021Benchmarking}. In contrast, the execution time significantly increases in more heavyweight data types, e.g., floating point data types, in which multiplication is software emulated in UPMEM PIM hardware~\cite{upmem-guide,Gomez2021Benchmarking}. Second, we observe that balancing the non-zero elements among tasklets typically outperforms balancing the rows for CSR/COO formats or blocks for BCSR/BCOO formats, since the non-zero element multiplications are computationally very expensive and can significantly affect load balance among tasklets. However, in delaunay\_n13 matrix, balancing the non-zero elements causes high row/block imbalance among tasklets, since one tasklet processes a significantly higher number of rows/blocks over the rest, thus incurring high operation imbalance among tasklets within the DPU core pipeline. As a result, balancing the rows/blocks outperforms balancing the non-zero elements due to the particular pattern of delaunay\_n13 matrix, and additionally performance improvements in BCSR/BCOO formats are higher, because they operate in block granularity and incur higher loop control costs. Third, we find that the fine-grain locking approach (COO.nnz-lb-fg) performs similarly with the coarse-grain locking approach (COO.nnz-lb-cg). Please see also Appendix~\ref{sec:appendix-1DPU-BCOO}. This is because the critical section includes memory accesses to the local DRAM bank, which in UPMEM PIM hardware are serialized in the DMA engine of the DPU. Therefore, the fine-grain locking approach does not increase the execution parallelism over the coarse-grain locking approach, since concurrent accesses to MRAM are not supported in UPMEM PIM hardware. Finally, we observe that the lock-free approach (COO.nnz-lf) outperforms the lock-based approaches (COO.nnz-lb-cg, COO.nnz-lb-fg) in delaunay\_n13 matrix, especially in data types where multiplication is supported by hardware. In delaunay\_n13 matrix, one tasklet processes a much higher number of rows over the rest, i.e., it performs a much higher number of critical sections over the rest, thus lock-based approaches cause high operation imbalance (in terms of lock acquisitions/releases and memory instructions) in the DPU core pipeline. Instead, lock-free and lock-based approaches in BCOO format perform similarly, since this format operates in block granularity. Thus, the skew on the number of blocks among tasklets of BCOO format has lower costs than the skew on the number of rows among tasklets of COO format, and also lock acquisition/release costs are hidden due to BCOO's higher loop control costs within the critical section.
\jgl{Readability would benefit from different paragraphs.}





\begin{tcolorbox}
\noindent\textbf{OBSERVATION 1:} \\
\textit{Operation imbalance} in computations, loop control iterations, synchronization points, or memory accesses among threads of a PIM core can cause \textit{high performance overheads}. \jgl{Not well formulated observation.}
\end{tcolorbox}

\begin{tcolorbox}
\noindent\textbf{OBSERVATION 2:} \\
\textit{Fine-grain locking} approaches to parallelize critical sections which perform memory accesses to different DRAM memory locations cannot improve performance over a \textit{coarse-grain} locking approach, when the PIM hardware does not support \textit{concurrent accesses to DRAM memory}. \jgl{Recommendation: Support subarray level parallelism... or more banks per core.}
\end{tcolorbox}





%\subsection{\textbf{Performance Comparison of Compressed Matrix Formats in One DPU}}\label{1DPU-AllFrmts}
%\noindent{\textbf{Performance Comparison of Compressed Formats in One DPU.}}
\noindent{\textbf{Analysis of Compressed Matrix Formats on One Single DPU.}} Figure~\ref{fig:1DPU-scalability} shows the scalability of all compressed formats for int8 and dbl64 data types when balancing the non-zero elements among tasklets. \jgl{Here and also in the previous section, I am missing the reason why we run these experiments and show the results. First thing to do is to explain what the goal of an experiment is.}




\begin{figure}[H]
\centering
\includegraphics[width=.8\textwidth]{1DPU/exec_time_int8.pdf}
\includegraphics[width=.8\textwidth]{1DPU/exec_time_dbl64.pdf}
\vspace{-12pt}
\caption{Scalability of all compressed formats for int8 and dbl64 data types increasing the number of tasklets of a single DPU.}
\label{fig:1DPU-scalability}
\vspace{-14pt}
\end{figure}


We draw out three findings. First, we find that even though DPU supports 24 tasklets, the \spmv{} execution typically scales up to 16 tasklets, since the DPU pipeline is fully utilized. Second, we observe that in data types with hardware-supported multiplication operation (e.g., int8 data type), CSR achieves the highest scalability, since it provides a better balance between memory accesses and computations. In contrast, in floating point data types (e.g. dbl64 data type), the DPU is significantly bottlenecked by the expensive software-emulated multiplication operations, thus all formats scale similarly. Third, we observe that BCSR and BCOO formats outperform CSR and COO formats in matrices that exhibit a block pattern (raefsky4 and pkustk08), only when multiplication is supported by hardware (e.g., int8 data type). This is  because they exploit spatial and temporal locality in WRAM memory in the accesses of the elements of the input vector. Instead, in dbl64 data type, performance is severely bottlenecked by computation, thus BCSR/BCOO perform worse than CSR/COO, since they incur higher indexing costs to discover the non-zero elements~\cite{asgari2020copernicus,Kanellopoulos2019SMASH}.
\jgl{No comments about the case/s where 24 performs better?}



\begin{comment}
%\begin{tcolorbox}
%\noindent\textbf{OBSERVATION 3:} \\
%\textit{High scalability} can be achieved if the compression format (e.g., CSR) effectively overlaps and balances memory accesses with computations in the core pipeline.
%\end{tcolorbox}
\end{comment}


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 3:} \\
Blocked formats (e.g., BCSR/BCOO) and can provide high performance gains over non-blocked formats (e.g., CSR/COO) in matrices that exhibit a block pattern, if the multiplication operation is supported by hardware. \jgl{How about other patterns?}
\end{tcolorbox}


==> backup/backup1/5-1D_2D.tex <==
%\section{Performance Characterization Among DPUs}
\section{Analysis of \spmv{} Execution on Multiple DPUs}


This section analyzes the \spmv{} execution using multiple DPUs in UPMEM PIM system. Section~\ref{Dataset} presents the matrix dataset. Section~\ref{1D} and Section~\ref{2D} evaluate 1D and 2D partitioning techniques, respectively \jgl{Give more information. How?}. Section~\ref{1D-2D} compares the 1D and 2D partitioning techniques. 





\subsection{Sparse Matrix Dataset}\label{Dataset}
We select 22 representative sparse matrices from Sparse Suite Collection~\cite{davis2011florida}, the characteristics of which are shown in Table~\ref{tab:large-matrices}. We highlight in red color matrices with a block pattern~\cite{Kourtis2011CSX,Elafrou2018SparseX}, and present the sparsity of the matrix (i.e., NNZ / (rows x columns)), the standard deviation of non-zero elements among rows (NNZ-r-std) and columns (NNZ-c-std). When the value of the last two metrics is high \jgl{Higher than what?}, the matrix is irregular~\cite{Namashivayam2021Variable,Tang2015Optimizing}, henceforth refer to as \textit{scale-free} matrix. Please see also Appendix~\ref{sec:appendix-matrix-dataset} for a complete description of our dataset of large sparse matrices.




% Flops / byte = (2 * nnz) / (8 * nnz + 12 * N), N : matrix dimension
% source: https://github.com/Sable/fait-maison-spmv
% Flops / byte = (2 * nnz) / (sizeof(datatype) * nnz + 12 * N), N : matrix dimension
\begin{table}[H]
\begin{center}
\vspace{-3mm}
\centering
\begin{minipage}{.48\linewidth}
%\resizebox{1.0\linewidth}{0.13\textheight}{
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|l|r|r|r|}
    \toprule
    \textbf{Matrix Name} & \textbf{Sparsity} & \textbf{NNZ-r-std} & \textbf{NNZ-c-std} \\
    \midrule
    \midrule
    hugetric-00020 (\textbf{hgc}) & 4.21e-07 & 0.031 & 0.031 \\ \hline 
    
    mc2depi (\textbf{mc2}) & 7.59e-06 & 0.076 & 0.076 \\ \hline 
    
    parabolic\_fem (\textbf{pfm}) & 	1.33e-05 & 0.153 &  0.153 \\ \hline 
    
    roadNet-TX (\textbf{rtn}) & 	1.98e-06 &  1.037 & 1.037 \\ \hline 
    
    rajat31 (\textbf{rjt})  &  9.24e-07  & 1.106  & 1.106 \\ \hline 
    
    \textcolor{darkred}{af\_shell1 (\textbf{ash})} & 	6.90e-05 & 1.275 & 1.275 \\ \hline  
    
    delaunay\_n19 (\textbf{del}) & 	1.14e-05 &  1.338 & 1.338 \\ \hline 
    
    thermomech\_dK  (\textbf{tdk}) & 6.81e-05 & 1.431 &  1.431 \\ \hline
    
    memchip	(\textbf{mem}) & 	2.02e-06 &  2.062 & 1.173 \\ \hline 
        
    amazon0601	(\textbf{amz}) & 	2.08e-05 &  2.79 & 15.29  \\ \hline 
    
    FEM\_3D\_thermal2 (\textbf{fth}) & 	1.59e-04 & 4.481  & 4.481 \\ \hline 

    \bottomrule
\end{tabular}
}
\end{minipage} \hspace{2pt}% 
\begin{minipage}{.48\linewidth}
%\resizebox{1.0\linewidth}{0.12\textheight}{
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{|l|r|r|r|}
    \toprule
    %\textbf{Matrix Shape} & \textbf{Matrix Name} & \textbf{Rows x Columns} & \textbf{NNZs} & \textbf{density} & \textbf{NNZ-r-std} & \textbf{NNZ-c-std} \\
    \textbf{Matrix Name} & \textbf{Sparsity} & \textbf{NNZ-r-std} & \textbf{NNZ-c-std} \\
    \midrule
    \midrule
    %\includegraphics[width=0.2\textwidth]{large_matrices/rajat31.png} & rajat31 & 4690002 x 4690002 & 20316253 & 0.0000009236 \\ \hline
     
    web-Google (\textbf{wbg}) & 	6.08e-06 & 6.557 &  38.366 \\ \hline
    
    \textcolor{darkred}{ldoor (\textbf{ldr})} & 	5.13e-05  & 11.951 & 11.951 \\ \hline 
    
    poisson3Db (\textbf{psb}) & 	3.24e-04  & 14.712  & 14.712 \\ \hline 
    
    \textcolor{darkred}{boneS10 (\textbf{bns})}  & 	6.63e-05 &  20.374 &  20.374 \\ \hline 
    
    webbase-1M (\textbf{wbs}) & 	3.106e-06 & 25.345  & 36.890 \\ \hline  
    
    in-2004	(\textbf{in}) & 	8.846e-06  & 37.230 & 144.062 \\ \hline 
    
    \textcolor{darkred}{pkustk14 (\textbf{pks})} & 	6.428e-04 &  46.508  & 46.508 \\ \hline  
    
    com-Youtube (\textbf{cmb}) & 4.639e-06  & 50.754  & 50.754 \\ \hline 

    
    sx-stackoverflow (\textbf{sxw}) & 	5.352e-06 &  137.849 & 65.367 \\ \hline 
    
    as-Skitter (\textbf{skt})  & 	7.71e-06  & 136.861 &  136.861 \\ \hline 
    
    ASIC\_680k (\textbf{ask})  & 	8.303e-06  & 659.807 & 659.807 \\ \hline 
 
    \bottomrule
\end{tabular}
}
\end{minipage}%
\end{center}
\caption{Matrix Dataset. Matrices are sorted on their irregular pattern (NNZ-r-std, NNZ-c-std metrics). \jgl{They are sorted by "r".}}
\label{tab:large-matrices}
\vspace{-20pt}
\end{table}



%\subsection{Performance Characterization of 1D Partitioning Techniques}\label{1D}
\subsection{Analysis of \spmv{} Execution Using 1D Partitioning Techniques}\label{1D}
We evaluate the 1D partitioning techniques highlighted in bold in Table~\ref{table:library}. Specifically, for COO.nnz, we evaluate the coarse-grain locking (COO.nnz-lb) and lock-free (COO.nnz-lf) approaches, since the fine-grain locking approach performs similarly with the coarse-grain locking approach, as shown in the previous section. For BCSR (int8 data type) and BCOO, we present the coarse-grain locking approach, since all synchronization approaches perform similarly, according to our evaluation of the previous section. Finally, in all experiments presented henceforth, we use 16 tasklets and select balancing the non-zero elements among tasklets within the DPU, since this load balancing scheme provides the highest performance benefits in the most common scenario, according to our evaluation shown in the previous section.



%\subsubsection{\textbf{Performance Characterization of Kernel Time.}}\label{1D-Kernel}
\subsubsection{\textbf{Analysis of Kernel Time.}}\label{1D-Kernel}
We compare the actual kernel time of \spmv{} achieved by various load balancing schemes for each particular compressed format, and then we compare the compressed formats between them.



\noindent\textbf{Analysis of Load Balancing Techniques Among DPUs.}
Figure~\ref{fig:1D_balance} compares load balancing techniques for each compressed format using 2048 DPUs and int32 data type. We draw out four findings. First, we observe that CSR.nnz and COO.nnz-rgrn, i.e., balancing the non-zero elements among DPUs (row granularity), either outperform or perform similarly to CSR.row and COO.row, respectively, i.e., balancing the rows among DPUs, apart from hgc and del matrices \jgl{Use special fonts for versions and matrices names.}. In these two matrices, CSR.nnz and COO.nnz-rowgrn incur a high skew in rows assigned to DPUs, i.e., only one DPU processes $4\times$ and $11\times$ more rows than the rest, for hgc and del matrices, respectively. This in turn creates a high skew in the elements of the output vector processed among DPUs, thus performance is limited by the DPU that processes the highest number of rows incurring high overheads. Thus, adaptive load balancing approaches and selection methods based on the characteristics of each particular matrix need to be developed. %to provide best performance across all matrices. 
Second, we find that COO.nnz-lb and COO.nnz-lf, which provide an almost perfect non-zero element balance among DPUs, significantly outperform COO.row and COO.nnz-rgrn in \textit{scale-free} matrices. Scale-free matrices have a few rows, which include a much higher number of non-zero elements over the remaining rows of the matrix. Thus, perfectly balancing the non-zero elements among DPUs provides high performance gains. Third, we find the lock-free COO.nnz-lf scheme outperforms the lock-based COO.nnz-lb scheme by 1.34$\times$ on average, and it provides high performance benefits when there is a high row imbalance among tasklets within DPU. When one tasklet processes a much higher number of rows over the rest, it executes a much higher number of critical sections, and the core pipeline incurs high imbalance in lock acquisitions/releases, thus the lock-based approach incurs high performance overheads in relatively compute-bound DPUs~\cite{Gomez2021Benchmarking}. Finally, in BCSR and BCOO, balancing the blocks is on average only slightly better than balancing the non-zero elements. 
\jgl{Divide into paragraphs and show the observation boxes after the corresponding paragraph.}





\begin{figure}[H]
\vspace{-14.6pt}
\centering
\begin{minipage}{\textwidth}
\includegraphics[width=.492\textwidth]{1D-partitioning/csr_balance_dpu_2048_int32.pdf}
\includegraphics[width=.492\textwidth]{1D-partitioning/coo_balance_dpu_2048_int32.pdf}
\end{minipage} % 
\begin{minipage}{\textwidth}
\includegraphics[width=.492\textwidth]{1D-partitioning/bcsr_balance_dpu_2048_int32.pdf}
\includegraphics[width=.492\textwidth]{1D-partitioning/bcoo_balance_dpu_2048_int32.pdf}
\end{minipage} 
\vspace{-10pt}
\caption{Performance comparison of load balancing techniques for each particular compressed format using 2048 DPUs and int32 data type. Matrices are sorted on their irregular pattern.}
\label{fig:1D_balance}
\vspace{-12pt}
\end{figure}


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 4:} \\
\textit{Perfectly balancing the non-zero elements} among PIM cores can provide significant performance benefits in \textit{highly irregular, scale-free matrices.}
\end{tcolorbox}

\begin{tcolorbox}
\noindent\textbf{OBSERVATION 5:} \\
\textit{Adaptive} load balancing schemes and selection methods for the balancing scheme on rows/blocks/non-zero elements based on the characteristics of the particular matrix need to be developed to provide best performance across all matrices.
\end{tcolorbox}

\begin{tcolorbox}
\noindent\textbf{OBSERVATION 6:} \\
\textit{Lock-free} approaches can provide high performance benefits over lock-based approaches in PIM architectures which typically include processors with relatively low compute throughput.
\end{tcolorbox}



Figure~\ref{fig:1D_datatypes} compares load balancing schemes in all data types. We present the geometric mean of all matrices using 2048 DPUs. In CSR and COO, balancing the non-zero elements among DPUs on average outperforms balancing the rows among DPUs. We observe that in COO format almost perfectly balancing the non-zero elements among DPUs provides significant performance benefits than balancing the number of rows, especially when multiplication is not supported by hardware (e.g., floating point types). Instead, in BCSR and BCOO, balancing the number of blocks among DPUs performs on average across all data types only slightly better than balancing the non-zero elements \jgl{How much is "slightly"? You should give numbers. This comment applies everywhere}.



\begin{figure}[H]
\begin{minipage}{\textwidth}
\centering
\includegraphics[width=.42\textwidth]{1D-partitioning/csr_datatypes_all_2048.pdf} \hspace{10pt}
\includegraphics[width=.42\textwidth]{1D-partitioning/coo_datatypes_all_2048.pdf} 
\end{minipage} 

\begin{minipage}{\textwidth}
\centering
\includegraphics[width=.42\textwidth]{1D-partitioning/bcsr_datatypes_all_2048.pdf} \hspace{10pt}
\includegraphics[width=.42\textwidth]{1D-partitioning/bcoo_datatypes_all_2048.pdf}
\end{minipage}  
\vspace{-12pt}
\caption{Performance comparison of load balancing techniques for each data type using 2048 DPUs.}
\label{fig:1D_datatypes}
\end{figure}



%\noindent\textbf{Comparison of Compressed Matrix Formats.}
\noindent\textbf{Analysis of Compressed Matrix Formats.}
Figure~\ref{fig:1D_kernel} compares the throughput (GOperations per second) achieved by various compressed formats using 2048 DPUs and int32 data type. For CSR and COO formats, we select balancing the non-zero elements, and for BCSR and BCOO formats, we select balancing the number of blocks, since these are the best-performing schemes for each format on average across all matrices and data types.

%the best-performing load balancing technique for the most common scenario. 



\begin{figure}[H]
    %\vspace{-1pt}
    \centering
    \includegraphics[width=\textwidth]{1D-partitioning/all_ops_kernel_dpus2048_int32-crop.pdf}
    \vspace{-10pt}
    \caption{Performance comparison of compressed formats using 2048 DPUs in int32 data type.}
    \label{fig:1D_kernel}
    \vspace{-14pt}
\end{figure}



We draw out three findings. First, matrices with block pattern (e.g., ash, ldr, bns, pks matrices) achieve the highest throughput, since they leverage higher data locality compared to matrices with non-block pattern. Second, we find that in scale-free matrices, COO and BCOO significantly outperform CSR and BCSR, respectively. This is because they provide better non-zero element balance among DPUs. In CSR and BCSR formats, the non-zero element balance provided is performed and is limited by row and block-row granularity, respectively. Moreover, we observe that BCOO can outperform CSR even in \textit{non-blocked} scale-free matrices. Finally, we find that when CSR and BCSR provide sufficient non-zero element balance among DPUs, e.g., in many regular matrices \jgl{Which ones?}, they can outperform COO and BCOO, respectively.


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 7:} \\ 
In scale-free matrices using an 1D partitioning approach, COO and BCOO formats significantly outperform CSR and BCSR formats, because they provide higher non-zero element balance among PIM cores.
\end{tcolorbox}



%\subsubsection{\textbf{End-to-end Performance Characterization.}}\label{1D-EndToEnd}
\subsubsection{\textbf{Analysis of End-To-End \spmv{} Performance.}}\label{1D-EndToEnd}
Figure~\ref{fig:1D_transfers} shows the total time of the best-performing 1D partitioning kernels using 2048 DPUs and int32 data type. The times are broken down into (i) the time for CPU to DPU transfer to load the input vector in MRAM banks (\textit{load}), (ii) the kernel time on DPUs (\textit{kernel}), (iii) the time for DPU to CPU transfer to retrieve the results for the output vector (\textit{retrieve}), and (iv) the time to merge partial results on the host CPU cores (\textit{merge}). 


\begin{figure}[H]
    \centering
    \includegraphics[width=.995\textwidth]{1D-partitioning/transfers_dpus2048_int32.pdf}
    \vspace{-10pt}
    \caption{Total execution time achieved when using 2048 DPUs and int32 data type for CR: CSR.nnz, CO:  COO.nnz-lf, BR: BCSR.block and BO: BCOO.block kernels.}
    \label{fig:1D_transfers}
\end{figure}


We draw out four findings. First, the load data transfers constitute more than 90\% of the total time, because the input vector is replicated and broadcasted at each DPU, thus a high amount of bytes is transferred through the narrow off-chip memory bus. An exception is in CSR and BCSR formats for sxw, ask matrices, which include one very dense row, thus kernel time is highly bottlenecked by one DPU that processes a significantly higher number of non-zero elements over the rest. Second, the kernel time constitutes on average only 4.3\% of the total time, since \spmv{} is effectively parallelized to thousand DPUs. Third, the retrieve data transfers constitute on average 3.4\% of the total time, because the output vector is split across DPUs. Finally, the reduce time on the host CPU is negligible (less than 1\% of the total time), since only a few partial results for the elements of the output vector are merged by the host CPU cores in the 1D partitioning techniques.


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 8:} \\
The end-to-end performance of the 1D partitioning technique is severely bottlenecked by the data transfer costs to replicate and broadcast the whole input vector at each DRAM bank of \textit{each} PIM core, which take place through the narrow off-chip memory bus.
\end{tcolorbox}




%To further investigate the costs of load data transfers, we present in 
Figure~\ref{fig:1D_transfers_scalability} shows the total time achieved by COO.nnz-lf when varying (a) the data type using 2048 DPUs, and (b) the number of DPUs for int32 data type. We draw two conclusions. First, the load data transfer costs increase proportionally to the number of bytes of the data type, and still dominate performance even for the data type with the smallest memory footprint (int8). Second, the load data transfer costs and the associated memory footprint for the input vector increase proportionally to the number of DPUs used, thus the best end-to-end performance is achieved using only a small portion of the available DPUs on the system. 


\begin{figure}[H]
    %\vspace{-1pt}
    \includegraphics[width=.7\textwidth]{1D-partitioning/transfers_datatypes_dpus2048.pdf}
    \includegraphics[width=.7\textwidth]{1D-partitioning/transfers_scalability_int32.pdf}
    \vspace{-10pt}
    \caption{End-to-end time breakdown achieved by COO.nnz-lf when varying (a) the data type using 2048 DPUs, and (b) the number of DPUs for int32 data type.}
    \label{fig:1D_transfers_scalability}
\end{figure}


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 9:} \\
The \spmv{} execution of the 1D partitioning schemes cannot scale up to a high number of PIM cores due to high data transfer overheads to copy the input vector at each DRAM bank of PIM-enabled memory.
%High data transfer overheads to copy the input vector at each DRAM bank limit the scalability of the 1D partitioning technique to a high number of PIM cores.
\end{tcolorbox}

\jgl{In general, I am quite lost in all this evaluation section. I think the main problem is that I don't get why all these experiments (because it is not clearly stated).}




%\subsection{Performance Characterization of 2D Partitioning Techniques}\label{2D}
\subsection{Analysis of \spmv{} Execution Using 2D Partitioning Techniques}\label{2D}
We evaluate 2D partitioning kernels highlighted in bold in Table~\ref{table:library}. Specifically, for COO we use the lock-free scheme, and for BCSR (int8 data type) and BCOO, we use the coarse-grain locking scheme. For BCSR and BCOO, in \equallyWidth{} and \variableSized{} techniques, we balance the number of blocks among DPUs of the same vertical partition, since it performs slightly better than balancing the non-zero elements, according to the previous section \jgl{What section? Are the conclusions from 1D applicable here?}. In all experiments, we balance the non-zero elements among 16 tasklets within DPU.



\subsubsection{\textbf{Analysis of Fine-grain Data Transfers.}}\label{2D-FineGrainTransfers}
\jgl{Where have we explained what we call coarse-grain or fine-grain data transfers?}
The UPMEM API~\cite{upmem-guide} requires transfer sizes at multiple DRAM banks \textit{to be of the same size}, and provides \textit{parallel transfers} either among all DPUs of all ranks, or in a rank granularity, i.e., among 64 DPUs of the same rank. Therefore, in \equallyWidth{} and \variableSized{} techniques, where the heights and widths of the 2D tiles vary, padding with empty bytes is necessary for the load and retrieve data transfers of the input and output vector, respectively. Figure~\ref{fig:2D_fgtransfers} compares coarse-grain transfers, i.e., performing parallel transfers across all 2048 DPUs, with fine-grain transfers, i.e., iterating over all ranks and performing parallel transfers among DPUs of the same rank, in \equallyWidth{} and \variableSized{} techniques using the COO format and having 2 and 32 vertical partitions. Please see Appendix~\ref{sec:appendix-2D-fgtrans} for all matrices.
 
 


\begin{figure}[H]
    \vspace{-8pt}
    \centering
    \includegraphics[width=.7\textwidth]{2D-partitioning/trans_reduced_dpus2048_int32_cps2.pdf}
    \includegraphics[width=.7\textwidth]{2D-partitioning/trans_reduced_dpus2048_int32_cps32.pdf}
    \vspace{-10pt}
    \caption{Performance comparison of RC: rbdcoo with coarse-grain transfers, RY: rbdcoo with fine-grain transfers in the output vector, BC: bdcoo with coarse-grain transfers, BY: bdcoo with fine-grain transfers only in the output vector, and BT: bdcoo with fine-grain transfers in both the input and the output vector using int32 data type, 2048 DPUs and having 2 (left) and 32 (right) vertical partitions.}
    \label{fig:2D_fgtransfers}
\end{figure}




We draw out two findings. First, when the number of vertical partitions is small, e.g., 2 vertical partitions, the widths among tiles in the \variableSized{} scheme only slightly vary, and the heights among tiles in \equallyWidth{} and \variableSized{} schemes highly vary \jgl{Slightly, highly... how much?}. Thus, BT and BY perform similarly, since a small amount of padding is added on the input vector in BY. Instead, RY and BY significantly outperform RC and BC, respectively, because fine-grain transfers on the output vector significantly decrease the amount of bytes transferred from PIM-enabled memory to host CPU. Second, when the number of vertical partitions is high, e.g., 32 vertical partitions, the heights among tiles in \equallyWidth{} and \variableSized{} schemes vary less compared to a small number of vertical partitions, and the widths among tiles in \variableSized{} scheme vary more \jgl{Vary less, vary more...}. Thus, RY and BY provide smaller performance benefits over RC and BC, respectively, compared to a small number of vertical partitions. Moreover, BT does not significantly outperforms BY, since fine-grain transfers on the input vector improve the \textit{load} time, which however constitutes only a small portion of the total time thanks to a high number of vertical partitions.


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 10:} \\ 
Fine-grain parallel transfers in \equallyWidth{} and \variableSized{} partitioning techniques to retrieve the elements of the output vector to host CPU can provide large performance gains. \jgl{The goal of these observation boxes is that someone reads them and understands the paper without reading the text. Make sure this is possible everywhere (it is not now).}
\end{tcolorbox}


%\subsubsection{\textbf{End-to-end Performance Characterization.}}\label{2D-EndToEnd}
\subsubsection{\textbf{Analysis of End-to-end Performance.}}\label{2D-EndToEnd}
In all experiments presented henceforth, we evaluate the end-to-end performance performing fine-grain transfers (rank granularity). %Please also see Appendix~\ref{sec:appendix-2D-scale}.




%\noindent\textbf{Comparison of Compressed Formats.}
\noindent\textbf{Analysis of Compressed Formats.}
Figure~\ref{fig:2D_balance} compares the performance of compressed matrix formats in 2D data partitioning techniques using 2048 DPUs \jgl{Do we ever show scaling on different DPU numbers? I think we are missing something important here: it may not make sense going for more DPUs if that means much more load time.} and int32 data type and having 4 vertical partitions. See Appendix~\ref{sec:appendix-2D-formats} for the complete evaluation using all 22 large matrices. We draw out two findings. First, we find that in \equallySized{} schemes, the kernel time is limited by the DPU (or a few DPUs) assigned to the 2D tile that includes the highest number of non-zero elements. In scale free matrices (e.g., in, ask) the deviation on the number of non-zero elements among 2D tiles is higher than regular matrices (e.g., pfg, bns), thus kernel time affects more the total execution time. Second, we find that CSR and BCSR perform worse than COO and BCOO (especially in \equallyWidth{} and \variableSized{} schemes) due to higher kernel time. In CSR and BCSR, data partitioning among DPUs or among tasklets within DPU is performed and limited \jgl{Avoid passive tense} by row and block-row granularity, respectively. Thus, these formats can cause higher non-zero imbalance among tasklets within DPU in \equallySized{} scheme, and both among DPUs and among tasklets within DPU in \equallyWidth{} and \variableSized{} schemes, compared to COO and BCOO formats. Overall, we find that COO and BCOO formats outperform CSR and BCSR in the most common scenarios \jgl{What are common scenarios?}, because they can provide parallelization schemes with high non-zero element balance among the processing units.




\begin{figure}[H]
    \centering
    \includegraphics[width=.7\textwidth]{2D-partitioning/fixed_time_reduced_norm_dpus2048_int32_cps4.pdf}
    \includegraphics[width=.7\textwidth]{2D-partitioning/rbal_time_reduced_norm_dpus2048_int32_cps4.pdf}
    \includegraphics[width=.7\textwidth]{2D-partitioning/bal_time_reduced_norm_dpus2048_int32_cps4.pdf}
    \vspace{-10pt}
    \caption{End-to-end time breakdown of 2D partitioning techniques for CR: CSR, CO: COO, BR: BCSR and BO: BCOO compressed matrix formats using 4 vertical partitions and int32 data type. \jgl{The colors of the plots look too uniform. Do they print ok in B/W? How about using some textures?} \jgl{(a), (b), (c) to describe the plots help to understand.}}
    \label{fig:2D_balance}
\end{figure}

\jgl{General comment: Revise the plots. "Time breakdown" is not what the y-axis of Fig. 13 shows. It shows execution time (in ms?). The breakdown itself is shown by the bars, not the y-axis.}


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 11:} \\
The kernel time in \equallySized{} schemes is limited by the PIM core (or a few PIM cores) assigned to the 2D tile with the highest number of non-zero elements. 
\end{tcolorbox}
\vspace{-4pt}

\begin{tcolorbox}
\noindent\textbf{OBSERVATION 12:} \\
The compressed matrix format used determines the data partitioning, thus affecting the load balance among PIM cores (and among threads within a multithreaded PIM core) with the corresponding performance implications.
\end{tcolorbox}



\noindent\textbf{Exploration on the Number of Vertical Partitions.}
Figure~\ref{fig:2D_vertpartitions} evaluates the performance of 2D partitioning techniques using COO format, when varying the number of vertical partitions from 1 to 32. We draw out four findings. First, in \equallySized{} scheme, as the number of vertical partitions increases, kernel time increases, if there is not one very dense row in the matrix. This is because the deviation on the non-zero elements among tiles increases with the increase on the number of vertical partitions, thus performance is limited by one (or a few) DPU that processes the highest number of non-zero elements. Second, as the number of vertical partitions increases, retrieve data transfer costs and merge time increase, since the partial results created for the output vector increase proportionally to the number of vertical partitions. The performance overheads of the retrieve data transfer costs are highly affected by the characteristics of the underlying hardware (e.g., the bandwidth provided on I/O channels of memory bus between host CPU and PIM-enabled DIMMs). Similarly, the performance cost of merge step depends on the characteristics of the host CPU (e.g., number of CPU cores and the available hardware threads, microarchitecture of CPU cores). Third, we find that in \equallyWidth{} and \variableSized{} schemes, there is high deviation on the heights of 2D tiles, and as a result on the number of partial results created among DPUs. Even with fine-grain retrieve parallel transfers in rank granularity, the amount of padding of the \equallyWidth{} and \variableSized{} schemes is  88.6\% and 88.0\% \jgl{Aren't serial transfers better in these cases?}, respectively, causing high bottlenecks in the narrow bus. Therefore, we find that in PIM systems that do not support fine-grain parallel transfers on gathering partial results from PIM-enabled DIMMs \textit{at DRAM bank granularity}, the execution is highly limited by the amount of padding performed in retrieve data transfers, which is typically high in irregular workloads like the \spmv{} kernel. Finally, we find that the number of vertical partitions which provides the best performance depends on the sparsity pattern of the matrix, the data type, the number of DPUs, and underlying hardware parameters (e.g., off-chip memory bus bandwidth, transfer latency costs between main memory and PIM-enabled memory, characteristics and microarchitecture of host CPU cores that perform merge step). In this work, we leave the exploration of selection methods on the the number of vertical partitions that provide best \spmv{} execution for future work. Overall, based on our analysis we conclude that the parallelization scheme that achieves the best performance in \spmv{} depends on both the sparse matrix given, and the hardware characteristics of the PIM system.



\begin{figure}[H]
    \centering
    \begin{minipage}{\textwidth}
    \centering
    \includegraphics[width=.7\textwidth]{2D-partitioning/fixed_vertical_dpus2048.pdf}
    \includegraphics[width=.7\textwidth]{2D-partitioning/rbal_vertical_dpus2048.pdf}
    \includegraphics[width=.7\textwidth]{2D-partitioning/bal_vertical_dpus2048.pdf}
    \end{minipage}
    \vspace{-10pt}
    \caption{Time breakdown of 2D partitioning schemes using COO format and 2048 DPUs when varying the number of vertical partitions from 1 to 32 for int8 and dbl64 data types. \jgl{What is the x-axis? Revise plots.}}
    \label{fig:2D_vertpartitions}
\end{figure}





\begin{tcolorbox}
\noindent\textbf{OBSERVATION 13:} \\
As the number of vertical partitions increases, the \equallySized{} scheme typically increases the non-zero element deviation among PIM cores (unless there is one dense row on the matrix), thus increasing the kernel time. 
\end{tcolorbox}


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 14:} \\
The \equallyWidth{} and \variableSized{} schemes require fine-grain parallel transfers at DRAM bank granularity to be supported by the system to achieve high performance.
\end{tcolorbox}

\begin{tcolorbox}
\noindent\textbf{OBSERVATION 15:} \\
There is no one-size-fits-all parallelization approach for \spmv{} in PIM systems, since the performance of each particular parallelization scheme depends on the characteristics of the input given and the underlying PIM hardware.
\end{tcolorbox}


\noindent\textbf{Scalability of 2D Partitioning Techniques}
%Figures~\ref{fig:2D_scale_four_parittions} and ~\ref{fig:2D_scale_sixteen_parittions}  present a scalability analysis to the number of DPUs for the 2D partitioning techniques using the COO format and having 4 and 16 vertical partitions, respectively.
\jgl{I do not understand why scalability is not evaluated earlier.}

Figures~\ref{fig:2D_scale_equally_sized}, ~\ref{fig:2D_scale_equally_wide} and ~\ref{fig:2D_scale_variable_sized}  present a scalability analysis to the number of DPUs for the 2D partitioning techniques using the COO format and for the \equallySized{}, \equallyWidth{} and \variableSized{} partitioning schemes, respectively.


\begin{figure}[H]
    \vspace{-6pt}
    \centering
    \begin{minipage}{\textwidth}
    \includegraphics[width=.48\textwidth]{2D-partitioning/scalability_fix_int32_col4.pdf}
    \includegraphics[width=.48\textwidth]{2D-partitioning/scalability_fix_int32_col16.pdf}
    \end{minipage}
    \vspace{-10pt}
    \caption{Time breakdown of \equallySized{} partitioning techniques of COO format using 4 (left) and 16 (right) vertical partitions when varying the number of DPUs used for int32 data type.}
    \label{fig:2D_scale_equally_sized}
    \vspace{-6pt}
\end{figure}


\begin{figure}[H]
    \vspace{-6pt}
    \centering
    \begin{minipage}{\textwidth}
    \includegraphics[width=.48\textwidth]{2D-partitioning/scalability_rbal_int32_col4.pdf}
    \includegraphics[width=.48\textwidth]{2D-partitioning/scalability_rbal_int32_col16.pdf}
    \end{minipage}
    \vspace{-10pt}
    \caption{Time breakdown of \equallyWidth{} partitioning techniques of COO format using 4 (left) and 16 (right) vertical partitions when varying the number of DPUs used for int32 data type.}
    \label{fig:2D_scale_equally_wide}
    \vspace{-6pt}
\end{figure}


\begin{figure}[H]
    \vspace{-6pt}
    \centering
    \begin{minipage}{\textwidth}
    \includegraphics[width=.48\textwidth]{2D-partitioning/scalability_bal_int32_col4.pdf}
    \includegraphics[width=.48\textwidth]{2D-partitioning/scalability_bal_int32_col16.pdf}
    \end{minipage}
    \vspace{-10pt}
    \caption{Time breakdown of \variableSized{} partitioning techniques of COO format using 4 (left) and 16 (right) vertical partitions when varying the number of DPUs used for int32 data type.}
    \label{fig:2D_scale_variable_sized}
    \vspace{-6pt}
\end{figure}



We draw out two findings. First, the \equallySized{} scheme achieves high scalability with a high number of vertical partitions. With a high number of \textit{static} vertical partitions the non-zero element deviation among DPUs is high, i.e., the kernel time is bottleneck by the DPU that processes the highest number of non-zero elements, thus increasing the number of DPUs improves performance by decreasing the kernel time via higher non-zero element balance among DPUs. %Instead, with a smaller number of vertical partitions kernel time of \equallySized{} scheme scales as the number of DPU increases mainly in \textit{scale-free} matrices (e.g., sxw and ask matrices), where there is high non-zero element deviation among DPUs due to their highly irregular pattern. 
Second, we observe that the \equallyWidth{} and \variableSized{} schemes are severely bottlenecked by retrieve data transfer costs (a high number of partial results is created on PIM-enabled DIMMs), thus they are hard to scale up to thousand DPUs. Moreover, when the number of vertical partitions is high, the deviation on the heights of the tiles is high, thus as the number of DPUs increases the amount of padding needed in retrieve data transfers becomes very high and severely degrades performance.



\begin{tcolorbox}
\noindent\textbf{OBSERVATION 16:} \\
The scalability of 2D partitioning techniques to a high number of PIM cores is severely limited by high data transfer overheads to retrieve partial results for the elements of the output vector created from DRAM banks to host CPU via the narrow memory bus.
%High data transfer overheads to retrieve partial results for the elements of the output vector created from DRAM banks  limit the scalability of the 2D partitioning techniques to a high number of PIM cores.
\end{tcolorbox}


\jgl{I am completely lost (and bored) at this point. The fact that there is no explanation or reasoning about the order of experiments, no clear goals for the experiments, etc. makes everything too painful to read.}



\noindent\textbf{Comparison of 2D Partitioning Techniques.}
Figure~\ref{fig:2D_best_partition} compares the throughput of 2D partitioning kernels using COO and BCOO formats and 2048 DPUs, since these two formats provide higher non-zero element balance in the most common scenario. For each kernel, we vary the number of vertical partitions from 2 to 32, with a step of power of 2, and select the best-performing execution. We draw out three findings. First, similarly to 1D partitioning kernels, matrices with block pattern (e.g., ash, ldr, bns, pks) achieve the highest throughput. Second, the \equallyWidth{} and \variableSized{} kernels perform similarly. Even though the \variableSized{} technique improves the non-zero element balance among DPUs and thus the kernel time over the \equallyWidth{} technique in most executions, the total time does not improve. In UPMEM PIM system, the performance of both techniques is severely bottlenecked by data transfer overheads due to a high amount of padding needed to retrieve partial results from PIM-enabled DIMMs to host CPU. Finally, we find that the \equallySized{} technique outperforms the \equallyWidth{} and \variableSized{} techniques in UPMEM PIM system, because it achieves lower data transfer overheads. The \equallyWidth{} and \variableSized{} techniques improve the non-zero element balance among DPUs, however sacrificing data transfer costs. As a result, we believe that a \textit{relaxed} \equallyWidth{} or \variableSized{} partitioning technique could be developed to provide a more relaxed non-zero element balance among DPUs, aiming to trade-off the non-zero element balance with the data transfer costs. 




\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{2D-partitioning/2d_ops_dpus2048_int32.pdf}
    \vspace{-10pt}
    \caption{Comparison of 2D partitioning kernels using COO and BCOO with 2048 DPUs for int32 type.}
    \label{fig:2D_best_partition}
\end{figure}



\subsection{Comparison of 1D and 2D Partitioning Techniques}\label{1D-2D}
Figure~\ref{fig:2D_1D-2D} compares 1D and 2D partitioning techniques. For 1D partitioning, we use the lock-free COO and lock-based BCOO kernels. For each matrix, we vary the number of DPUs from 64 to \dpuActive{}, and select the best-performing end-to-end execution. For 2D partitioning, we use the \equallySized{} COO and BCOO kernels with \dpuActive{}. For each matrix, we vary the number of vertical partitions from 2 to 32 (step of power of 2), and select the best-performing end-to-end execution. 


\begin{figure}[H]
    %\vspace{-1pt}
    \centering
    \includegraphics[width=\textwidth]{2D-partitioning/1d-2d_ops_dpus2528_flt32-crop.pdf}
    \vspace{-10pt}
    \caption{Throughput achieved by 1D and 2D partitioning techniques for flt32 data type. \jgl{From the plot, I do not know what is 1D and what is 2D.}}
    \label{fig:2D_1D-2D}
\end{figure}





We draw two conclusions. First, we observe that the best performance is achieved using a much smaller number of DPUs than the available DPUs on the system. In 1D partitioning kernels (i.e., COO.nnz-lf and BCOO.block), replicating the input vector at a high number of DPUs significantly increases the load transfer costs. Thus, across all matrices, best performance is achieved using less than 512 DPUs. In 2D partitioning kernels (i.e., dcoo, dbcoo), creating \equallySized{} 2D tiles incurs high non-zero element deviation among tiles, and many tiles are empty, i.e., do not include any non-zero element. Thus, across all matrices, best performance is achieved using less than 1200 DPUs, because DPUs associated at empty tiles are idle. Second, we find that in regular matrices, the 2D partitioning kernels outperform the 1D partitioning kernels, because they use a higher number of DPUs, thus kernel time is lower. In contrast, in scale-free matrices, the 2D partitioning kernels perform worse than the 1D partitioning kernels, because the \equallySized{} technique significantly increases the non-zero element deviation among DPUs, i.e., kernel time is bottlenecked by only one (or a few) DPU that processes a much higher number of non-zero elements compared to the rest, thus kernel time is higher.


\begin{tcolorbox}
\noindent\textbf{OBSERVATION 17:} \\
Expensive data transfers to PIM-enabled memory performed via the narrow memory bus impose significant performance overhead to the end-to-end \spmv{} execution, thus it is hard to fully exploit all available PIM cores of the system.
\end{tcolorbox}

\jgl{After so much text, plots and observations, I have only two conclusions: (1) the slowest DPU determines the time, (2) data transfers are very slow.}

\jgl{I think there is a problem with the motivation and logical order of experiments, which affects the whole flow.}


==> backup/backup1/6-cpu_gpu.tex <==

\section{Comparison with CPUs and GPUs}\label{cpu-gpu}

We compare the \spmv{} execution in UPMEM PIM system with \dpuActive{}, to an Intel Xeon CPU and an NVIDIA Tesla V100 GPU, the characteristics of which are shown in Table~\ref{tab:cpu-gpu}. We use peakperf~\cite{peak-perf} and stream~\cite{stream} for CPU and GPU systems to calculate peak performance, bandwidth, and TDP. For UPMEM PIM, we estimate the peak performance as $Total\_DPUs * AT$, where arithmetic throughput (AT) is shown in Appendix~\ref{sec:appendix-1DPU-AT}, the total bandwidth as $Total\_DPUs * Bandwidth\_DPU$, where the Bandwidth\_DPU is 700MB/s~\cite{Gomez2021Benchmarking,devaux2019}, and TDP as $(Total\_DPUs / DPUs\_per\_chip) * 1.2W/chip$ from prior work~\cite{Gomez2021Benchmarking,devaux2019}.



\begin{table}[H]
\begin{center}
\centering
\resizebox{1.0\linewidth}{0.04\textheight}{
\begin{tabular}{lccccccc}
    \toprule
    \textbf{System} & \textbf{Process Node} & \textbf{Total Cores} & \textbf{Frequency} & \textbf{Peak Performance} & \textbf{Memory Capacity} & \textbf{Total Bandwidth} & \textbf{TDP} \\
    \midrule
    Intel Xeon Silver 4110 (2 sockets) & 14nm & 2x8 cores (2x16 threads) & 2.1GHz & 660 GFLOPS & 128GB & 23.1GB/s  & 2x85W \\ \hline 
    NVIDIA Tesla V100 & 12nm & 5120 cuda cores & 1.25GHz & 14.13 TFLOPS & 32GB & 897GB/s & 300W \\ \hline 
    PIM System & 2x nm & \dpuActive{} & 350MHz & 4.66 GFLOPS & 159GB & 1.77TB/s & 379W \\ \hline 

    \bottomrule
\end{tabular}
}
\end{center}
\caption{Evaluated CPU, GPU, and UPMEM PIM Systems. \jgl{The table looks bad. Check the aspect ratio (same for tables in the appendix).}}
\label{tab:cpu-gpu}
\end{table}




For CPU system, we use the optimized CSR kernel from TACO library~\cite{Kjolstad2017Taco}. For GPU system, we use CSR5 CUDA~\cite{Weifeng2015CSR5,CSR5-cuda} for int32 data type and cuSparse~\cite{cuSparse} for the other data types. For UPMEM PIM system, we use the lock-free COO 1D partitioning kernel (\textbf{COO}.nnz-lf) and the \equallySized{} COO kernel (\textbf{DCOO}). In the former, we run experiments from 64 up to \dpuActive{}, and in the latter, we use \dpuActive{}, and vary the number of vertical partitions from 2 to 32 with a step or power of 2. In both kernels, we select the best-performing end-to-end execution. We also include the lock-free COO 1D partitioning kernel using \dpuActive{}, named \textbf{COO.kl}, to evaluate the performance executing \spmv{} split to all available DPUs of the system.



Figure~\ref{fig:cpu-gpu-end_to_end} shows the throughput of \spmv{} (in GOperations per second) in all systems, comparing both the end-to-end time (i.e., including the load and retrieve transfer costs for the input and output vectors in case of UPMEM PIM and GPU systems), and only the actual kernel time (i.e., including the kernel time in DPUs and merge time in host CPU for UPMEM PIM system). We draw three conclusions. First, when data transfer costs to/from host CPU are included, CPU performs best, since data transfers impose high overhead. When only the actual kernel time is considered, GPU performs best, since it is the system that provides the highest compute throughput, i.e., 14.13 TFlops. Second, we evaluate the portion of the peak performance achieved by \spmv{} in all systems, and observe that \spmv{} in UPMEM PIM system \spmv{} performs the closest to its peak performance compared to CPU and GPU. For flt32 data type, \spmv{} achieves on average 0.51\% and 0.21\% of the peak performance in CPU and GPU, respectively, while it achieves 51.7\% of the peak performance in UPMEM PIM system. Achieving a high portion of the peak performance is highly desirable, because it means that the software highly exploits the computation capabilities of the underlying hardware. This way it improves the processor/resource utilization, and the cost of ownership of the underlying hardware. Finally, we also observe that when all DPUs are used, i.e., COO.kl execution, UPMEM PIM outperforms the CPU by 1.09$\times$ and 1.25$\times$ for int8 and int32 data types, the multiplication of which is supported by hardware, and performs 1.27$\times$ and 2.39$\times$ worse than CPU for flt32 and dbl64 data types, the multiplication of which is software emulated in DPUs. 



\begin{figure}[t]
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_perf_dpus2528_int8.pdf}\hspace{12pt}
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_perf_dpus2528_int32.pdf}
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_perf_dpus2528_flt32.pdf}\hspace{12pt}
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_perf_dpus2528_dbl64.pdf}
    \vspace{-4pt}
    \caption{Performance comparison between the UPMEM PIM sytem, Intel Xeon CPU and Tesla V100 GPU.}
    \label{fig:cpu-gpu-end_to_end}
\end{figure}



\begin{tcolorbox}
\noindent\textbf{OBSERVATION 18:} \\
\spmv{} can perform significantly closer to the peak performance in real PIM architectures compared to processor-centric CPU and GPU systems, since PIM architectures mitigate data movement costs.
\end{tcolorbox}



For energy measurements, we consider only the actual kernel time in all systems (in UPMEM PIM we consider the kernel and merge steps). We use Intel RAPL~\cite{rapl} on the CPU, and NVIDIA SMI~\cite{smi} on the GPU. For UPMEM PIM, we measure the number of cycles, instructions, WRAM accesses and MRAM accesses of each DPU, and estimate energy with energy weights provided by UPMEM company~\cite{upmem}. Figure~\ref{fig:cpu-gpu-energy} shows the energy consumption (in Joules) and performance per energy unit (in GOps/W) in all systems. We draw out three findings. First, GPU provides the largest energy savings over the other two systems, since  the energy results follow the performance results. Second, we find that the 2D partitioning kernel (DCOO) consumes more energy than the 1D partitioning kernels (COO, COO.kl), because of the energy consumed in host CPU. CPU cores merge a high number of partial results in 2D partitioning kernels to assemble the final output vector, thus increasing the energy consumption. Finally, we find that the 1D partitioning kernels provide larger energy savings over the CPU system for int8 and int32 data types (3.16$\times$ and 4.52$\times$, respectively), and better performance per energy unit (1.74$\times$ and 1.14$\times$, respectively).





\begin{figure}[t]
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_energy_dpus2528_int8.pdf}\hspace{12pt}
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_energy_dpus2528_int32.pdf}
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_energy_dpus2528_flt32.pdf}\hspace{8pt}
    \includegraphics[width=.4\textwidth]{cpu-gpu/cpu-gpu_energy_dpus2528_dbl64.pdf}
    \vspace{-10pt}
    \caption{Energy comparison between the UPMEM PIM system, Intel Xeon CPU and Tesla V100 GPU. \jgl{The plots would benefit from getting rid of the little points that are outliers. All Energy plots would be much more clear.}}
    \label{fig:cpu-gpu-energy}
\end{figure}



\begin{tcolorbox}
\noindent\textbf{OBSERVATION 19:} \\
Real PIM architectures can provide high energy-efficiency on \spmv{}, when multiplication operation is supported by hardware. \jgl{I don't get this. Isn't int32 multiplication emulated?}
\end{tcolorbox}





\noindent\textbf{\textit{Discussion.}}
These observations are useful for programmers to anticipate how much performance and energy savings they can get on \spmv{} from UPMEM PIM hardware compared to traditional CPU and GPU systems. However, our proposed \SparseP{} library can be adapted and evaluated at other current and future real PIM systems with potentially higher compute capabilities and energy-efficiency than UPMEM PIM system. Moreover, one limitation to ensure fair comparison among three types of systems is that hardware characteristics, such as fabrication technology, process node, number of cores, or frequency (Table~\ref{tab:cpu-gpu}) are very different across the three systems. The UPMEM PIM system have comparable memory capacity to the CPU. On the other hand, GPU has much lower memory capacity than UPMEM PIM system, and its cost is much higher than UPMEM PIM system. We also note that the UPMEM hardware is still maturing and is expected to run at a higher frequency in the near future (500 MHz instead of 350 MHz) and potentially be manufactured with a smaller technology node~\cite{upmem,Gomez2021Benchmarking}. Hence, the results we report in this comparison may underestimate the full potential of the UPMEM-based PIM architecture.
\jgl{What is this discussion? Isn't it copied from my paper? That is not good.}
\jgl{You are analyzing a single application. You can be more specific about what needs to be done for PIM to outperform CPUs and GPUs.}




==> backup/backup1/7-takeaways.tex <==


\section{Key Takeaways and Recommendations}

This section summarizes our key takeaways in the form of recommendations to improve multiple aspects of PIM hardware and software.


\noindent\textbf{\textit{Recommendation \#1.}} \textit{Design algorithms that provide high balance among threads of PIM core in terms of computations, loop control iterations, synchronization points and memory accesses.} 
Section~\ref{1DPU} shows that high skew on rows (or blocks), non-zero elements, lock acquisitions/releases or memory accesses among multiple threads on \spmv{} can impose high overhead in a compute-bound PIM core~\cite{Gomez2021Benchmarking}. From a programmer’s perspective, the architecture requires a shift in how we optimize parallel programs, since high operation balance is vital for multithreaded PIM cores.



\noindent\textbf{\textit{Recommendation \#2.}} \textit{Design compressed data structures that can be effectively partitioned across DRAM banks targeting to provide high computation balance among PIM cores.} Sections~\ref{1D-Kernel} and ~\ref{2D-EndToEnd} show that CSR and BCSR formats perform significantly worse over COO and BCOO formats on \spmv{}, since they incur high non-zero element imbalance among PIM cores. This is because the matrix is stored in row- or block-row order for CSR and BCSR, respectively, thus data partitioning across DRAM banks is limited by row- or block-row granularity, respectively. Therefore, we suggest programmers to design compressed data structures that can provide effective data partitioning schemes with high computation balance among multiple PIM cores.




\noindent\textbf{\textit{Recommendation \#3.}} \textit{Design \textit{adaptive} algorithms that both strive a balance between computation and data transfer costs, and adapt their configuration to the particular patterns of each input given, as well as the characteristics of the PIM hardware.} Our analysis on Sections~\ref{1D-Kernel} and~\ref{2D-EndToEnd} demonstrates that best-performing \spmv{} execution on UPMEM PIM system can be achieved using algorithms that (i) trade off computation and data transfer costs, and (ii) select the load balancing strategy and data partitioning policy on the particular sparsity pattern of the input matrix. In addition, the load balancing scheme and data partitioning technique that provides the best throughput in \spmv{} execution depends on the characteristics of the underlying PIM system (See Section~\ref{2D-EndToEnd}). To this end, we recommend software designers to implement heuristics and selections methods to adapt their algorithms on the underlying hardware characteristics of the PIM system and the particular characteristics of the given input.





\noindent\textbf{\textit{Recommendation \#4.}} \textit{Provide low-cost synchronization support and concurrent accesses to DRAM bank to increase parallelism on a multithreaded PIM core.} Section~\ref{1DPU} shows that lock acquisitions/releases can be very expensive in the DPU pipeline, and fine-grain locking approaches to parallelize critical sections do not improve performance over a coarse-grain approach (critical sections are serialized), since UPMEM PIM hardware serializes MRAM accesses in the DMA engine. Based on this key takeaway, we recommend hardware designers to provide lightweight synchronization mechanisms~\cite{Giannoula2021SynCron} for multithreaded PIM cores, and enable concurrent access to local DRAM memory arrays to increase execution parallelism.


 

\noindent\textbf{\textit{Recommendation \#5.}} \textit{Optimize the broadcast collective operation in data transfers from main memory to PIM-enabled memory to minimize overheads of copying the input data at all DRAM banks.} Figure~\ref{fig:1D_transfers} shows that the 1D partitioning technique on \spmv{} is severely limited by data transfers to copy the input vector at \textit{each} DRAM bank of PIM cores, which take place through the narrow off-chip memory bus. Thus, we recommend hardware and system designers to provide a fast broadcast collective primitive to DRAM banks of PIM-enabled memory.




\noindent\textbf{\textit{Recommendation \#6.}} \textit{Optimize the gather collective operation \textit{at DRAM bank granularity} for data transfers from PIM-enabled memory to host CPU to minimize overheads of retrieving the output results.} Figure~\ref{fig:2D_vertpartitions} demonstrates that the \equallyWidth{} and \variableSized{} 2D partitioning techniques are severely limited by data transfers to retrieve partial results for the elements of the output vector from DRAM banks of PIM-enabled DIMMs. This is because a high amount of padding is needed (on average 88.3\%) to perform parallel transfers at a rank granularity (64 DPUs). Therefore, we suggest hardware and system designers to provide an optimized gather collective and fine-grain parallel transfers \textit{at DRAM bank granularity} (i.e., having variable transfer sizes across DRAM banks) from PIM-enabled memory to host CPU.




\noindent\textbf{\textit{Recommendation \#7.}} \textit{Design high-speed communication channels and optimized libraries for data transfers to/from  DRAM banks of PIM-enabled memory.} Section~\ref{cpu-gpu} demonstrates that \spmv{} execution on a real PIM system achieves a much higher fraction of the peak performance (on average 51.7\% for float data type), compared to processor-centric CPU and GPU systems. However, the end-to-end performance is significantly limited by data transfer costs on the narrow memory bus. To this end, we recommend that the hardware architecture and the software stack be enhanced with support for low-cost and fast data transfers to/from PIM-enabled memory modules.


==> backup/backup1/8-related_work.tex <==


\section{Related Work}

To our knowledge, this is the first work that (i) extensively characterizes the \spmv{} kernel in a real PIM system, and (ii) presents an \spmv{} library for real PIM systems. We discuss prior work.



\noindent\textbf{Sparse Matrix Kernels in PIM Systems.} Xie et al.~\cite{Xie2021SpaceA} design heterogenous PIM units to accelerate \spmv{} in HMC-based PIM systems. Fujiki et al.~\cite{Fujiki2019Near} enhance the memory controllers of GPUs with PIM cores to on-the-fly transform the matrix from CSR to DCSR format~\cite{Changwan2018Efficient} to minimize memory traffic. Zhu et al.~\cite{Zhu2013Accelerating} propose a PIM accelerator for Sparse Matrix Matrix Multiplication. These works propose hardware designs for sparse matrix kernels, while our work studies software optimizations to accelerate the \spmv{} execution on real PIM systems. 



\noindent\textbf{\spmv{} in Commodity Systems.} Numerous prior works propose optimized \spmv{} algorithms for CPUs~\cite{Elafrou2018SparseX,Buluc2011Reduced,Elafrou2017PerformanceAA,Kjolstad2017Taco,Merrill2016Merge,Willcock2006Accelerating,Williams2007Optimization,Namashivayam2021Variable,Tang2015Optimizing,Elafrou2019Conflict}, GPUs~\cite{Bolz2003Sparse,Hong2018Efficient,Liu2014AnEfficient,Wu2010Efficient,Yan2014YaSpMV,Guo2014APerformance,Choi2010Model,su2012ClSpMV,Yan2014YaSpMV,Steinberger2017Globally,Shengen2014YaSpMV}, heterogeneous CPU-GPU systems~\cite{Yang2017Hybrid,Indarapu2014Architecture,Yang2015Performance,Benatia2020Sparse} systems, and distributed CPU systems~\cite{Lee2008Adaptive,Bisseling2005Communication,Bylina2014Performance,Page2018Scalability,Kayaaslan2015Semi,Liu2018Towards}. Optimized \spmv{} kernels for processor-centric CPU and GPU systems exploit shared memory model of these systems and data locality in deep cache hierarchies. However, these kernels  cannot be directly mapped in most near-bank PIM systems, which have a distributed memory model, and shallow cache hierarchies. Most well-tuned \spmv{} kernels for distributed CPU and CPU-GPU systems improve performance by overlapping computation with communication among processing units. Instead, real near-bank PIM architectures are fundamentally different than commodity systems, since they are highly-distributed, include a shallow memory hierarchy, and typically there is no direct communication among PIM cores. Thus, \spmv{} kernels designed for common processor-centric systems, cannot be directly applied to near-bank PIM systems.



\noindent\textbf{Compressed Matrix Formats.} Prior works propose a range of compressed formats~\cite{Im1999Optimizing,Langr2016Evaluation,Liu2015CSR5,Pinar1999Improving,Vuduc2005Fast,Yang2014Optimization,Yan2014YaSpMV,Kourtis2011CSX,Kourtis2008Optimizing,Kourtis2008Optimizing,Belgin2009Pattern,LIL,ELL,bjorck1996numerical,Pooch1973Survey,Shubhabrata2007Scan,Changwan2018Efficient}, and selection methods to find the most efficient format~\cite{su2012ClSpMV,Niu2021TileSpMV,asgari2020copernicus,Zhao2018Overhead,Sedaghati2015Automatic,Benatia2016Sparse,Zhao2018Bridging,Li2013SMAT,Maggioni2013AdELL,Tan2018Design,Li2015Performance,Benatia2018BestSF}. In this work, we have extensively explored the four most widely used formats, and observe that the compressed format: (i) needs to provide good balance among computation and memory accesses inside the core pipeline, and (ii) affects load balancing among PIM cores with the corresponding performance implications. Thus, some compressed formats designed for commodity processor-centric systems might not be suitable for real PIM systems. We leave the exploration of other PIM-suitable formats for future work.



\noindent\textbf{Hardware Accelerators for \spmv{}.} Recent works design accelerators for \spmv{}~\cite{Sadi2019Efficient,Fowers2014AHigh,Grigoras2015Accelerating,Lin2010Design,Umuroglu2014Anenergy,Kanellopoulos2019SMASH,Mukkara2018Exploiting}, or other sparse kernels~\cite{Asgari2020Alrescha,Hegde2019ExTensor,Zhang2016CambriconX,Pal2018OuterSpace,Nurvitadhi2016Hardware,Eric2020sigma}. Instead, our work proposes software optimizations, and provides the first characterization study of \spmv{} in a real PIM system.







==> backup/backup1/9-conclusion.tex <==


\section{Conclusion}
We  present \SparseP{}, the first open-source \spmv{} library for real PIM systems, and conduct the first comprehensive characterization analysis of \spmv{} in a real commercial PIM architecture. We explore the four most widely used compressed matrix formats, various load balancing approaches and synchronization schemes among threads of a multithreaded PIM core. We provide 1D and 2D data partitioning techniques to map \spmv{} on thousand PIM cores to optimize its end-to-end execution time. We analyze various \spmv{} kernels in a wide variety of sparse matrices with diverse sparsity patterns and characteristics using the first real commercial PIM architecture. Finally, we compare the performance and energy of \spmv{} on a PIM system to a state-of-the-art CPU and GPU systems to estimate the potential of the \spmv{} execution on a real PIM system over conventional processor-centric architectures. Our extensive evaluation of \SparseP{} library provides programming recommendations for software designers, and suggestions and hints for hardware and system designers of future PIM systems. We believe and hope that our work will provide valuable insights to programmers designing software implementations of memory-bound kernels (apart from the \spmv{} kernel), and architects of this PIM architecture as well as of future PIM systems, and will represent an enabling milestone in the adoption and commercialization of near-bank PIM systems.
